Quantum Distributed Algorithms for Detection of Cliques

The possibilities offered by quantum computing have drawn attention in the distributed computing community recently, with several breakthrough results showing quantum distributed algorithms that run faster than the fastest known classical counterparts, and even separations between the two models. A prime example is the result by Izumi, Le Gall, and Magniez [STACS 2020], who showed that triangle detection by quantum distributed algorithms is easier than triangle listing, while an analogous result is not known in the classical case. In this paper we present a framework for fast quantum distributed clique detection. This improves upon the state-of-the-art for the triangle case, and is also more general, applying to larger clique sizes. Our main technical contribution is a new approach for detecting cliques by encapsulating this as a search task for nodes that can be added to smaller cliques. To extract the best complexities out of our approach, we develop a framework for nested distributed quantum searches, which employ checking procedures that are quantum themselves. Moreover, we show a circuit-complexity barrier on proving a lower bound of the form $\Omega(n^{3/5+\epsilon})$ for $K_p$-detection for any $p \geq 4$, even in the classical (non-quantum) distributed CONGEST setting.

==> CCSection_-_Copy.tex <==
%======================================
% \section{A \qclique algorithm for detecting $K_p$}
\section{The Power of Nested Quantum Search: Detection from Listing in the Quantum Congested Clique}
\label{sec:CC}
%======================================
\rtodo{Re-write intro text after final structure is settled}
In this section we describe two approaches that take an algorithm for $K_p$-listing in the \clique or \qclique model,
and extend it into an algorithm for $K_{p+t}$-freeness (for some $t > 0$).
The first approach yields somewhat slower algorithms, but it has 
the advantage of taking 
the $K_p$-listing algorithm \emph{as a black box} (i.e., any $K_p$-listing algorithm can be used, including sparsity-aware algorithms, etc.).
This approach also forms the basis for our $\CONGEST$ algorithms in Section \ref{sec:qcongest}.

The second approach yields faster algorithms, but it 
``opens the black box'': it explicitly uses the $K_p$-listing algorithm from \cite{DLP12} and relies on its properties.

\subsection[Approach I: Extending $K_p$ \emph{listing} to $K_{p+t}$ \emph{detection}]{Approach I: Extending {\boldmath $K_p$} \emph{listing} to {\boldmath $K_{p+t}$} \emph{detection}}

Suppose that each $p$-clique in the input graph $G$ is known to some node of the clique, 
and we now want to check if the graph contains a $(p+1)$-clique.
Classically, we would have to consider every possible node $\tilde{v} \in V$,
and check whether it extends some known $p$-clique into a $(p+1)$-clique.
This translates to $n$ ``queries'', where each query check a specific node $\tilde{v} \in V$.
Using distributed Grover search, we can speed up this process, and perform only $O(\sqrt{n})$ ``quantum queries''.
Evaluating each query --- that is, checking whether a given node $\tilde{v} \in V$ extends some known $p$-clique into a $(p+1)$-clique --- is easy
in the congested clique: 
we simply ask every clique node $u \in V$ to inform all clique nodes whether or not $\set{u,\set{v}} \in E$.
This requires a single round, so the total running time of the entire search is $\tilde{O}(\sqrt{n})$ (by Lemma~\ref{lemma:qsearchv0}).

\paragraph{The initial state.}
When we begin our algorithm, we assume that we have already detected some copies of $K_p$ (possibly all, but not necessarily):
each node $v \in V$ has a subset $S_v^p \subseteq V^{(p)}$ \rtodo{notation for subsets of size $p$}
of $p$-cliques it has found, such that if $\set{ u_1,\ldots,u_p } \in S_v^p$
then $(u_1,\ldots,u_p)$ is indeed a copy of $K_p$ in $G$.
Let
\begin{equation*}
	S^p = \bigcup_{v \in V} S_v^p
\end{equation*}
be all the copies of $K_p$ detected by the nodes.
We say that an algorithm $A$ \emph{extends} from $K_p$ to $K_{p+t}$ if,
given sets $\set{ S_v^p }_{v \in V}$ as described above,
w.h.p., \rtodo{what does this mean formally --- introduce some convention in the preliminaries}
algorithm $A$ outputs '1' at all nodes
iff $G$ contains a $(p+t)$-clique $\set{ u_1,\ldots,u_{p+t} } \in V^{(p+t)}$ such that
$(u_1,\ldots,u_p) \in S^p$.

\newcommand{\ThmExtending}
{
	For every $p \geq 2$, $t \geq 1$,
	there is an algorithm that extends from $K_p$ to 
	$K_{p+t}$ in $\tilde{O}(n^{1-1/2^t})$ rounds in $\qclique$.
}

\begin{theorem}
	\label{extendingTheorem}
	\ThmExtending
\end{theorem}
%The proof is given in Appendix~\ref{app:CC}.


\begin{proof}

	The proof is by induction on $t$.

%\paragraph{Base case, $t= 1$.} 
\subparagraph{Base case, {\boldmath $t = 1$}.}
To check for the presence of a $(p+1)$-clique that extends one of the $p$-cliques
in $S^p$, we perform a Grover search over the nodes of the graph,
and for each $\tilde{u} \in V$, we describe a classical query $Q_{\tilde{u}}$ that checks whether 
$u$
forms a $(p+1)$-clique together with some $p$-clique in $S^p$.
The query $Q_{\tilde{u}}$ is carried out in a single communication round, \rtodo{This doesn't include reporting to the leader\dots} as follows:
\begin{itemize}
	\item Every node $v \in V$ broadcasts to the entire clique whether $\set{ \tilde{u},v} \in E$ or not.
	\item Locally, every node $v$ checks whether there is some $p$-clique $\set{ u_1,\ldots,u_p} \in S_v^p$
		that node $u$ extends into a $(p+1)$-clique:
		that is, node $v$ checks whether
		for each $i = 1,\ldots,p$ we have $\set{ \tilde{u}, u_i} \in E$.
\end{itemize}
Since we are searching over $n$ nodes and each query requires constant time,
by Lemma~\ref{lemma:qsearchv0},
the running time of the entire algorithm is $\tilde{O}( \sqrt{n} )$.

\subparagraph{Induction step.}
Suppose that for every $p \geq 2$,
there exists an algorithm $A_{t-1,p}$ that extends from $K_p$ to $K_{p+t-1}$.
Now fix a concrete $p \geq 2$, and let us describe an algorithm $A_{t,p}$ that extends from $K_p$ to $K_{p+t}$.

In $A_{t,p}$, we partition the nodes $V$ of the graph into batches $V_1,\ldots,V_{n^{1/2^{t-1}}}$,
each of size $n^{1-1/2^{t-1}}$ \rtodo{assuming it divides cleanly},
and perform a Grover search over the batches,
to check whether there exists a node $\tilde{u}_{p+1} \in V_i$
and nodes $\hat{u}_{p+2},\ldots,\hat{u}_{p+t} \in V$
that extend some known $p$-clique $\set{ u_1,\ldots,u_p} \in S_v$
into a $(p+t)$ clique, $\set{ u_1,\ldots,u_p, \tilde{u}_{p+1}, \hat{u}_{p+1},\ldots,\hat{u}_{p+t}}$.

The query $Q_i$ that evaluates the $i$-th batch $V_i$ is carried out as follows:
\begin{itemize}
	\item Each node $v \in V$ broadcasts, for each $\tilde{u}_{p+1} \in V_i$,
		whether $\set{ v , \tilde{u}_{p+1}} \in E$.
	\item Locally, each $v \in V$ creates a set $S_v^{p+1}$ of $(p+1)$-cliques 
		that extend some previously-known $p$-clique by adding a node from $V_i$:
		\begin{equation*}
			\set{ u_1,\ldots,u_{p}, \tilde{u}_{p+1}} \in S_v^{p+1}
			\quad
			\Leftrightarrow
			\quad
			\set{ u_1,\ldots,u_p} \in S_v^p \text{ and }
			\set{ u_1, \tilde{u}_{p+1}}, \ldots, \set{ u_p, \tilde{u}_{p+1}} \in E.
		\end{equation*}
	\item We execute the algorithm $A_{p+1, t - 1}$ with the sets $\set{ S_v^{p+1} }_{v \in V}$
		and return its answer.
\end{itemize}
The running time of $Q_i$ is $\tilde{O}(n^{1-1/2^{t-1}})$ rounds:
the first step requires $\tilde{O}(n^{1-1/2^{t-1}})$ rounds because $|V_i| = n^{1-1/2^{t-1}}$.
The second step also requires $\tilde{O}(n^{1-1/2^{t-1}})$, by the induction hypothesis.
Since we are searching over $n^{1/2^{t-1}}$ batches,
by Lemma~\ref{lemma:qsearchv1}


\subparagraph{Induction step.}
Suppose that the claim holds for all values up to $t - 1$, and let us prove it for $t$.
The idea is to first 

Assume correctness for all values up to $t$, exclusive.



We split $V$ into sets $V_{1}, \dots, V_{n^{1/2^{t-1}}}$, each of size $O(n^{1-1/2^{t-1}})$. We perform a Grover search over these sets. Fix $i \in [n^{1/2^{t-1}}]$, and observe $V_i$. As before, the node of the graph broadcast whether they neighbor each of the nodes in $V_i$, requiring $|V_i| = O(n^{1-1/2^{t-1}})$ rounds. Then, we execute the algorithm for extending $K_{p+1}$ to $K_{p + t}$, by using $\tilde{t} = t-1$, within $\tilde O(n^{1-1/2^{\tilde{t}}}) = \tilde O(n^{1-1/2^{t-1}})$ rounds. Finally, as we perform a Grover search over $i \in [n^{1/2^{t-1}}]$, where each checking step requires $\tilde{O}(n^{1-1/2^{t-1}})$ rounds, our algorithm completes in $\tilde{O}(n^{1/2^{t}} \cdot n^{1-1/2^{t-1}}) =  \tilde{O}(n^{1-1/2^t}) $ rounds.\vspace{2mm}

To see the correctness of the algorithm, assume that there exists some instance of $K_{p+t}$ denoted $\kappa_{p+t} = \{v_1, \dots, v_{p+t}\}$. Also denote $\kappa_{p} = \{v_1, \dots, v_{p}\}$ and $\kappa_{p+1} = \{v_1, \dots, v_{p+1}\}$. Observe that some node $w$ knows about $\kappa_p$, as this is given. Observe the set $V_i$ such that $v_{p+1} \in V_i$. When performing the Grover search and looking at $V_i$, node $w$ will become aware of $\kappa_{p+1}$ as all the nodes in $\kappa_p$ will inform $w$ that $v_{p+1}$ neighbors them. Then, when performing the algorithm for extending all \emph{known}\footnote{Note that, the algorithm detects the existence of an instance of $K_{p+t}$ which contains a \emph{known} instance of $K_p$, as a subgraph, where \emph{known} means that some node is aware of its existence. For brevity, in the statement of the theorem, we state that it is assumed all instances of $K_p$ are known.} $K_{p+1}$ to $K_{p + t}$, node $w$ will be made aware of $\kappa_{p+t}$.

%Suppose that every $p$-clique in the graph is known to some clique node,
%and we would like to check if the graph contains a $(p+1)$-clique, in $\tilde{O}(\sqrt{n})$ rounds.
%
%Given that every instance of $K_p$ is known to some node, we desire to detect if there is an instance of $K_{p+1}$ in the graph, within $\tilde O(n^{1/2})$ rounds.
%We perform a Grover search over the nodes, to look for a node $\tilde{v} \in V$ that forms a $(p+1)$-clique together with some $p$-clique that we have already found.
%To check a particular candidate $\tilde{v} \in V$, we ask all other nodes $u \in V$ to broadcast to the entire clique
%whether they are neighbors with $\tilde{v}$ or not. This requires only one round of communication,
%and subsequently, every clique node knows all of $\tilde{v}$'s edges. We now have every clique node locally check whether it knows of some $p$-clique $u_1,\ldots,u_p$ such that $\tilde{v}$ is a neighbor of all $p$ clique nodes.
%If such a clique is found, we announce that we have found a $(p+1)$-clique.
%
%The correctness of the algorithm follows from the fact that every $p$-clique is initially known to some clique node.
%If the graph contains a $(p+1)$-clique $u_1,\ldots,u_{p+1}$,
%then some clique node $w$ knows of the $p$-clique $u_1,\ldots,u_p$.
%When we evaluate the query for $u_{p+1}$, node $w$ will see that $u_{p+1}$ is a neighbor of $u_1,\ldots,u_p$,
%and will find the clique.
%
%The running time of the algorithm is $\tilde{O}(\sqrt{n})$, because we must perform $n$ quantum queries,
%and each query requires a single round to evaluate.

\end{proof}

Further, one can show a \emph{sparsity-aware} version of Theorem~\ref{extendingTheorem}. The key realization is that information regarding $\Theta(n)$ edges can be broadcast in the \clique model in $O(1)$ rounds, thus, enabling one to coalesce the checking of several nodes at once. This in turn changes the dependency of the round complexity from the number of nodes in the graph, $n$, to the average degree in the graph, $\mu = \Theta(m/n)$. 

\begin{theorem}
	\label{extendingTheoremSparsityAware}
	Given a graph $G = (V, E)$ and values $p$, $t$. Assuming that every instance of $K_p$ is known to some node, then it is possible to detect if $G$ contains an instance of $K_{p + t}$ in $\tilde{O}(\mu^{1-\frac{1}{2^t}})$ rounds of communication in the \qclique, w.h.p. 
\end{theorem}

\begin{proof}
	Initially, we \emph{batch} together the nodes into sets such that the sum of the degrees of the nodes in each set is $\Theta(n)$. Clearly, by broadcasting the degree of each node, it is possible to partition the nodes into $V = Y_1 \cup \dots \cup Y_{y}$, where, for $i \in [y]$ the sum of the degrees in $Y_i$ is $\Theta(n)$, and $y = \Theta(m/n) = \Theta(\mu)$. Thus, within $1$ round, all nodes can locally compute such a partition. 
	
	Further, observe that for any $i \in [y]$, it is possible in $O(1)$ rounds of the \clique to broadcast the neighbors of every node in $Y_i$. To do so, every node in $Y_i$ broadcasts its degree, allowing all the nodes to locally \emph{assign} to every node $O(1)$ of the edges  incident to nodes in $Y_i$. Finally, as every node is assigned $O(1)$ edges, it broadcasts those edges in $O(1)$ rounds.
	
	Similarly to the $Y_i$ sets, we split $V$ into sets $X_{1}, \dots, X_{x}$, where $x = \mu^{1/2^{t-1}}$, ensuring that the sum of the degrees on the nodes in each set is $\Theta(m/x)$. Notice that similarly to the above, it is possible to broadcast the edges incident to all nodes in a specific $X_i$ in $\Theta(m/[x\cdot n] = \mu / x)$ rounds.
	
	As in the proof of Theorem~\ref{extendingTheorem}, we prove by induction on $t$.\vspace{2mm}
	
%	\paragraph{Base case, $t= 1$.} 
\noindent{\bf Base case, {\boldmath $t= 1$}.}
Given that every instance of $K_p$ is known to some node, we desire to detect if there is an instance of $K_{p+1}$ in the graph, within $\tilde O(\mu^{1/2})$ rounds. To do so, we perform a Grover search over $y$, to look for $i \in [y]$ such that there exists $v^* \in Y_i$ where $v^*$ is in some instance of $K_{p+1}$. That is, fix $i \in [y]$, and, using the above, broadcast the edges incident to the nodes in $Y_i$. Then, every node broadcasts if it is aware of some $K_{p+1}$ or not. If there is a $\tilde{v} \in Y_i$ and an instance of $K_{p+1}$ which includes $\tilde{v}$, denoted $\kappa = \{v_1, \dots, v_p, \tilde{v}\}$, then it is guaranteed that some node knows it, due to similar claims as in the proof of Theorem~\ref{extendingTheorem}.
	% Denote by $w$ the node which knows the instance of $K_p$, $\kappa \setminus \{\tilde{v}\}= \{v_1, \dots, v_p\}$. It is guaranteed that such a $w$ exists as we are given that all $K_p$ have been listed. Thus, as the edges incident to the nodes in $Y_i$, and hence $\tilde{v}$ have been broadcast, node $w$ sees $\kappa$ and reports to the entire graph that a $K_{p+1}$ exists. 
	Finally, we perform this Grover search over $[y]$, and so due to Lemma~\ref{lemma:qsearch}, this executes in $\tilde O(y^{1/2})$ rounds.\vspace{2mm}
	
	
%	\paragraph{Induction step, assuming correctness for $<t$.}  
\noindent{\bf Induction step, assuming correctness for \boldmath{$<t$}.}
We perform a Grover search over the sets $X_1, \dots, X_{x}$. Recall that $x = \mu^{1/2^{t-1}}$. Fix $i \in [\mu^{1/2^{t-1}}]$, and observe $X_i$. As before, broadcast the edges incident to nodes in $X_i$ within $\Theta(\mu / x) = \Theta(\mu^{1-1/2^{t-1}})$ rounds. Then, execute the algorithm for extending $K_{p+1}$ to $K_{p + t}$, by using $\tilde{t} = t-1$, within $\tilde O(\mu^{1-1/2^{\tilde{t}}}) = \tilde O(\mu^{1-1/2^{t-1}})$ rounds. Finally, as we perform a Grover search over $i \in [\mu^{1/2^{t-1}}]$, where each checking step requires $\tilde{O}(\mu^{1-1/2^{t-1}})$ rounds, the algorithm completes in $\tilde{O}(\mu^{1/2^{t}} \cdot \mu^{1-1/2^{t-1}}) =  \tilde{O}(\mu^{1-1/2^t}) $ rounds.\vspace{2mm}
	
	The correctness of the algorithm follows exactly from the same claims as in the proof of Theorem~\ref{extendingTheorem}.
\end{proof} 

%To do so, we perform a Grover search over $V$, to look for a node $v^* \in V$ such that $v^*$ is in some instance of $K_{p+1}$. That is, fix $\tilde{v} \in V$, and every node $u \in V$ broadcasts if $\tilde{v}$ is its neighbor. Then, every node broadcasts if it is aware of some $K_{p+1}$ or not. If there is an instance of $K_{p+1}$ which includes $\tilde{v}$, denoted $\kappa = \{v_1, \dots, v_p, \tilde{v}\}$, then it is guaranteed that some node knows it. Denote by $w$ the node which knows the instance of $K_p$, $\kappa \setminus \{\tilde{v}\}= \{v_1, \dots, v_p\}$. It is guaranteed that such a $w$ exists as we are given that all $K_p$ have been listed. Thus, node $w$ would receive messages from each of $\kappa \setminus \{\tilde{v}\}$ telling it that they neighbor $\tilde{v}$, and so $w$ would see $\kappa$ and report to the entire graph that a $K_{p+1}$ exists. Finally, we perform this Grover search over $V$, and so due to Lemma~\ref{lemma:qsearch}, this executes in $\tilde O(n^{1/2})$ rounds.\vspace{2mm}

%\paragraph{Induction step, assuming correctness for $<t$.} 

%%%% NEW p -> p+t extension %%%%%%%%%%%%%%%%%
%\input{newccextend.tex}


==> app_CC.tex <==
\section{Missing Proofs from Section~\ref{sec:CC}}
\label{app:CC}

%\begin{theorem-repeat}{extendingTheorem}
	%\ThmExtending
%\end{theorem-repeat}
%
%\begin{proof}[Proof of Theorem~\ref{extendingTheorem}]
%
%We show this theorem by induction on $t$. 
%
%%\paragraph{Base case, $t= 1$.} 
%\subparagraph{Base case, {\boldmath $t = 1$}.}
%Suppose that every $p$-clique in the graph is known to some clique node,
%and we would like to check if the graph contains a $(p+1)$-clique, in $\tilde{O}(\sqrt{n})$ rounds.
%
%Given that every instance of $K_p$ is known to some node, we desire to detect if there is an instance of $K_{p+1}$ in the graph, within $\tilde O(n^{1/2})$ rounds.
%We perform a Grover search over the nodes, to look for a node $\tilde{v} \in V$ that forms a $(p+1)$-clique together with some $p$-clique that we have already found.
%To check a particular candidate $\tilde{v} \in V$, we ask all other nodes $u \in V$ to broadcast to the entire clique
%whether they are neighbors with $\tilde{v}$ or not. This requires only one round of communication,
%and subsequently, every clique node knows all of $\tilde{v}$'s edges. We now have every clique node locally check whether it knows of some $p$-clique $u_1,\ldots,u_p$ such that $\tilde{v}$ is a neighbor of all $p$ clique nodes.
%If such a clique is found, we announce that we have found a $(p+1)$-clique.
%
%The correctness of the algorithm follows from the fact that every $p$-clique is initially known to some clique node.
%If the graph contains a $(p+1)$-clique $u_1,\ldots,u_{p+1}$,
%then some clique node $w$ knows of the $p$-clique $u_1,\ldots,u_p$.
%When we evaluate the query for $u_{p+1}$, node $w$ will see that $u_{p+1}$ is a neighbor of $u_1,\ldots,u_p$,
%and will find the clique.
%
%The running time of the algorithm is $\tilde{O}(\sqrt{n})$, because we must perform $n$ quantum queries,
%and each query requires a single round to evaluate.
%
%\subparagraph{Induction step.}
%Assume correctness for all values up to $t$, exclusive.
%We split $V$ into sets $V_{1}, \dots, V_{n^{1/2^{t-1}}}$, each of size $O(n^{1-1/2^{t-1}})$. We perform a Grover search over these sets. Fix $i \in [n^{1/2^{t-1}}]$, and observe $V_i$. As before, the node of the graph broadcast whether they neighbor each of the nodes in $V_i$, requiring $|V_i| = O(n^{1-1/2^{t-1}})$ rounds. Then, we execute the algorithm for extending $K_{p+1}$ to $K_{p + t}$, by using $\tilde{t} = t-1$, within $\tilde O(n^{1-1/2^{\tilde{t}}}) = \tilde O(n^{1-1/2^{t-1}})$ rounds. Finally, as we perform a Grover search over $i \in [n^{1/2^{t-1}}]$, where each checking step requires $\tilde{O}(n^{1-1/2^{t-1}})$ rounds, our algorithm completes in $\tilde{O}(n^{1/2^{t}} \cdot n^{1-1/2^{t-1}}) =  \tilde{O}(n^{1-1/2^t}) $ rounds.\vspace{2mm}
%
%To see the correctness of the algorithm, assume that there exists some instance of $K_{p+t}$ denoted $\kappa_{p+t} = \{v_1, \dots, v_{p+t}\}$. Also denote $\kappa_{p} = \{v_1, \dots, v_{p}\}$ and $\kappa_{p+1} = \{v_1, \dots, v_{p+1}\}$. Observe that some node $w$ knows about $\kappa_p$, as this is given. Observe the set $V_i$ such that $v_{p+1} \in V_i$. When performing the Grover search and looking at $V_i$, node $w$ will become aware of $\kappa_{p+1}$ as all the nodes in $\kappa_p$ will inform $w$ that $v_{p+1}$ neighbors them. Then, when performing the algorithm for extending all \emph{known}\footnote{Note that, the algorithm detects the existence of an instance of $K_{p+t}$ which contains a \emph{known} instance of $K_p$, as a subgraph, where \emph{known} means that some node is aware of its existence. For brevity, in the statement of the theorem, we state that it is assumed all instances of $K_p$ are known.} $K_{p+1}$ to $K_{p + t}$, node $w$ will be made aware of $\kappa_{p+t}$.
%\end{proof}
%
%Further, one can show a \emph{sparsity-aware} version of Theorem~\ref{extendingTheorem}. The key realization is that information regarding $\Theta(n)$ edges can be broadcast in the \clique model in $O(1)$ rounds, thus, enabling one to coalesce the checking of several nodes at once. This in turn changes the dependency of the round complexity from the number of nodes in the graph, $n$, to the average degree in the graph, $\mu = \Theta(m/n)$. 
%
%\begin{theorem}
%	\label{extendingTheoremSparsityAware}
%	Given a graph $G = (V, E)$ and values $p$, $t$. Assuming that every instance of $K_p$ is known to some node, then it is possible to detect if $G$ contains an instance of $K_{p + t}$ in $\tilde{O}(\mu^{1-\frac{1}{2^t}})$ rounds of communication in the \qclique, w.h.p. 
%\end{theorem}
%
%\begin{proof}
%	Initially, we \emph{batch} together the nodes into sets such that the sum of the degrees of the nodes in each set is $\Theta(n)$. Clearly, by broadcasting the degree of each node, it is possible to partition the nodes into $V = Y_1 \cup \dots \cup Y_{y}$, where, for $i \in [y]$ the sum of the degrees in $Y_i$ is $\Theta(n)$, and $y = \Theta(m/n) = \Theta(\mu)$. Thus, within $1$ round, all nodes can locally compute such a partition. 
%	
%	Further, observe that for any $i \in [y]$, it is possible in $O(1)$ rounds of the \clique to broadcast the neighbors of every node in $Y_i$. To do so, every node in $Y_i$ broadcasts its degree, allowing all the nodes to locally \emph{assign} to every node $O(1)$ of the edges  incident to nodes in $Y_i$. Finally, as every node is assigned $O(1)$ edges, it broadcasts those edges in $O(1)$ rounds.
%	
%	Similarly to the $Y_i$ sets, we split $V$ into sets $X_{1}, \dots, X_{x}$, where $x = \mu^{1/2^{t-1}}$, ensuring that the sum of the degrees on the nodes in each set is $\Theta(m/x)$. Notice that similarly to the above, it is possible to broadcast the edges incident to all nodes in a specific $X_i$ in $\Theta(m/[x\cdot n] = \mu / x)$ rounds.
%	
%	As in the proof of Theorem~\ref{extendingTheorem}, we prove by induction on $t$.\vspace{2mm}
%	
%%	\paragraph{Base case, $t= 1$.} 
%\noindent{\bf Base case, {\boldmath $t= 1$}.}
%Given that every instance of $K_p$ is known to some node, we desire to detect if there is an instance of $K_{p+1}$ in the graph, within $\tilde O(\mu^{1/2})$ rounds. To do so, we perform a Grover search over $y$, to look for $i \in [y]$ such that there exists $v^* \in Y_i$ where $v^*$ is in some instance of $K_{p+1}$. That is, fix $i \in [y]$, and, using the above, broadcast the edges incident to the nodes in $Y_i$. Then, every node broadcasts if it is aware of some $K_{p+1}$ or not. If there is a $\tilde{v} \in Y_i$ and an instance of $K_{p+1}$ which includes $\tilde{v}$, denoted $\kappa = \{v_1, \dots, v_p, \tilde{v}\}$, then it is guaranteed that some node knows it, due to similar claims as in the proof of Theorem~\ref{extendingTheorem}.
%	% Denote by $w$ the node which knows the instance of $K_p$, $\kappa \setminus \{\tilde{v}\}= \{v_1, \dots, v_p\}$. It is guaranteed that such a $w$ exists as we are given that all $K_p$ have been listed. Thus, as the edges incident to the nodes in $Y_i$, and hence $\tilde{v}$ have been broadcast, node $w$ sees $\kappa$ and reports to the entire graph that a $K_{p+1}$ exists. 
%	Finally, we perform this Grover search over $[y]$, and so due to Lemma~\ref{lemma:qsearch}, this executes in $\tilde O(y^{1/2})$ rounds.\vspace{2mm}
%	
%	
%%	\paragraph{Induction step, assuming correctness for $<t$.}  
%\noindent{\bf Induction step, assuming correctness for \boldmath{$<t$}.}
%We perform a Grover search over the sets $X_1, \dots, X_{x}$. Recall that $x = \mu^{1/2^{t-1}}$. Fix $i \in [\mu^{1/2^{t-1}}]$, and observe $X_i$. As before, broadcast the edges incident to nodes in $X_i$ within $\Theta(\mu / x) = \Theta(\mu^{1-1/2^{t-1}})$ rounds. Then, execute the algorithm for extending $K_{p+1}$ to $K_{p + t}$, by using $\tilde{t} = t-1$, within $\tilde O(\mu^{1-1/2^{\tilde{t}}}) = \tilde O(\mu^{1-1/2^{t-1}})$ rounds. Finally, as we perform a Grover search over $i \in [\mu^{1/2^{t-1}}]$, where each checking step requires $\tilde{O}(\mu^{1-1/2^{t-1}})$ rounds, the algorithm completes in $\tilde{O}(\mu^{1/2^{t}} \cdot \mu^{1-1/2^{t-1}}) =  \tilde{O}(\mu^{1-1/2^t}) $ rounds.\vspace{2mm}
%	
%	The correctness of the algorithm follows exactly from the same claims as in the proof of Theorem~\ref{extendingTheorem}.
%\end{proof} 

%\subsection[Faster detection of $K_p$]{Faster detection of {\boldmath $K_p$}}


%Given Theorem~\ref{extendingTheorem}, we can show an algorithm for detection of $K_p$, which is faster than listing for $p \geq 5$.

%\begin{theorem}
	%Given a graph $G = (V, E)$, and some value $p$, it is possible to detect whether there exists an instance of $K_p$ in $G$ within $\tilde{O}(\min_{\ell \in \mathbb{N}} \max \{n^{1-\frac{2}{p-\ell}}, n^{1-\frac{1}{2^\ell}}\})$ rounds of the \qclique model.
%\end{theorem}

%For instance, using $p = 5$, and $\ell = 1$, we get $K_5$ detection in $\tilde O(n^{1/2})$ rounds of the \qclique model.

%\begin{proof}
	%Fix $\ell \in \mathbb{N}$. Perform $K_{p-\ell}$ listing using the algorithm from \cite{DLP12} within $\tilde O(n^{1-\frac{2}{p-\ell}})$ rounds. Then, execute Theorem~\ref{extendingTheorem} within $\tilde O(n^{1-1/2^{\ell}})$ rounds in order to detect the existence of an instance of $K_p$.
%\end{proof}

\iffalse
Using Theorem~\ref{extendingTheoremSparsityAware}, it is possible to show a sparsity aware version of the above.

\begin{theorem}
	Given a graph $G = (V, E)$, and some value $p$, it is possible to detect whether there exists an instance of $K_p$ in $G$ within $\tilde{O}(\min_{\ell \in \mathbb{N}} \max \{m / n^{1+\frac{2}{p-\ell}}, (m/n)^{1-\frac{1}{2^\ell}}\})$ rounds of the \qclique model.
\end{theorem}


\begin{proof}
	Fix $\ell \in \mathbb{N}$. Perform $K_{p-\ell}$ listing using the algorithm from \cite{CHLGL20} within $\tilde O(m/n^{1+\frac{2}{p-\ell}})$ rounds. Then, execute Theorem~\ref{extendingTheoremSparsityAware} within $\tilde O((m/n)^{1-1/2^{\ell}})$ rounds in order to detect the existence of an instance of $K_p$.
\end{proof}
\fi

\iffalse
\subsection{Missing Details from Section~\ref{sec:CCfast}}

\noindent{\bf Analyzing the runtime of the algorithm for extending from $K_p$ to $K_{p+t}$.}
We explain how to derive the values of the parameters $r_1,\ldots,r_t \in (0,1)$, which determine the runtime of the algorithm.
Recall that after the pre-processing stage, each node $v$ knows all the edges crossing between the sets $T_1^v,\ldots,T_p^v$,
which are each of size $n^{1-1/p}$.
We require for each $i = 1,\ldots,t$ that $1 - r_i \leq {1-1/p}$ (i.e., $r_i \geq 1/p$), as this ensures that the time required to learn 
the additional edges necessary for step $i$ of the recursion does not exceed the time required for the pre-processing stage (asymptotically).

Let $f(p,i)$ denote the running time of $\proc{check}_{p+i}(P_1,\ldots,P_{p+i}, F)$,
where $| \bigcup_{\ell = 1}^{p+i} P_i | = O( n^{1-1/p} )$ (recall that we think of $p,t$ as constants).
The number of edges a node needs to learn for the next step of the recursion (depth $i+1$)
is at most
\begin{equation*}
	O(n^{1-1/p} \cdot n^{1 - r_{i+1}} + n^{2(1 - r_{i+1})}) = O(n^{1-1/p + 1 - r_{i+1}}),
\end{equation*}
because $1 - r_{i+1} \leq 1-1/p$.
Using Lenzen routing~\cite{Lenzen13},
this can be done in $O(n^{1 - 1/p - r_{i+1}})$ rounds.
Therefore, %\TODO{This doesn't quite mesh with the new statement of the nested quantum search, because there we give all levels at once and here it's described level-by-level}
\begin{equation}
	f(p,i) = n^{r_{i+1} / 2} \cdot \left( c_{p,i} \cdot n^{1 - r_{i+1} - 1/p} + f(p, i+1)\right),
	\label{eq:recursion}
\end{equation}
where $c_{p,i}$ is some constant.

The recursion ends at depth $t$, where we perform a purely local computation, and hence $f(p,t) = 1$.
At each level $i < t$, we balance the setup cost --- that is, the cost of collecting the edges needed for the next recursion level --- against the cost of the recursive call: for some constant $\alpha_{p,i}$,
\begin{equation}
	\alpha_{p,i} = f(p,i) = c_{p,i} n^{1-1/p - r_{i}}.
	\label{eq:balance}
\end{equation}
Plugging~\eqref{eq:balance} into~\eqref{eq:recursion} yields
\begin{align*}
	f(p,i)
	&= 
	(\alpha_{p,i+1} + 1) n^{r_{i+1}/2} f(p, i+1)
	\\
	&=
	(\alpha_{p,i+1} + 1) (\alpha_{p,i+2} + 1)
	n^{r_{i+1}/2} n^{r_{i+2}/2} f(p, i+2)
	\\
	&= \ldots
	\\
	&=
	\prod_{\ell = i+1}^t (\alpha_{p,\ell} + 1)
	n^{\sum_{\ell = i+1}^{t} r_{\ell} / 2} f(p, t)
	=
	\prod_{\ell = i+1}^t (\alpha_{p,\ell} + 1)
	n^{\sum_{\ell = i+1}^{t} r_{\ell} / 2},
\end{align*}
where in the last step we use the fact that $f(p,t) = 1$.

Solving the recursion by working backwards from $i = t$ down to $i = 1$,
we obtain
\begin{equation*}
	r_{t-i} = \frac{1}{2^i}\left( 1 - \frac{1}{p} \right),
\end{equation*}
that is,
\begin{equation*}
	r_i = \frac{1}{2^{t-i}}\left( 1 - \frac{1}{p} \right).
\end{equation*}
For the running time, we get
\begin{align*}
	f(p,i) 
	&=
	\left( \prod_{\ell = i+1}^t (\alpha_{p,\ell} + 1) \right)
	n^{\sum_{\ell = i+1}^t (1/2^{t-\ell}) (1 - 1/p) / 2}
	\\
	&= 
	\left( \prod_{\ell = i+1}^t (\alpha_{p,\ell} + 1) \right)
	n^{((1 - 1/p) / 2)\sum_{j = 0}^{t-i-1} (1/2^{j}) }
	\\
	&= 
	\left( \prod_{\ell = i+1}^t (\alpha_{p,\ell} + 1) \right)
	n^{(1 - 1/p) (1-1/2^{t-i})},
\end{align*}
and in particular, for $i = 0$,
\begin{equation*}
	f(p,0) = O( n^{ (1 - 1/p)(1 - 1/2^{t}) } ).
\end{equation*}
We observe that this solution indeed satisfies~\eqref{eq:balance}:
the time required for the setup phase at depth $i$ is
\begin{equation*}
	c_{p,i} n^{1-1/p - r_i} = c_{p,i} n^{1-1/p - (1/2^{t-i})(1-1/p)}
	=
	c_{p,i} n^{(1-1/p)(1 - 1/2^{t-i})}
	,
\end{equation*}
and this indeed matches $f(p,i)$, for an appropriate choice of the constants $\alpha_{p,j}$.\vspace{2mm}


\noindent{\bf Formal statement of the algorithm as a nested quantum search.}
%\paragraph{Formal statement of the algorithm as a nested quantum search.}
Fix $p \geq 2$ and $t \geq 1$ satisfying the constraint.
Also, for each $i = 1,\ldots,t$,
fix a partition $X_i^1,\ldots,X_i^{n^{r_i}}$ of $V$,
where
$r_i = (1-1/p)/2^{t-i}$,
and $|X_i^1| = \ldots = |X_i^{n^{r_i}}| = n^{1-r_i}$.
The partitions are arbitrary, but fixed in advance, so no communication is necessary to compute them.
Note that $r_i \geq 1/p$ for each $i = 1,\ldots,t$.

Our algorithm is a depth-$t$ nested quantum search, over the search space 
$[ r_1 ] \times \ldots \times [r_t]$,
with the goal function $f : [ r_1 ] \times \ldots \times [r_t] \rightarrow \set{0,1}$
such that 
	$f(i_1,\ldots,i_t) = 1$
	iff
	there exists a $p$-clique $v_1,\ldots,v_p \in V^p$,
	and there exist $u_1 \in X_1^{i_1},\ldots,u_t \in X_t^{i_t}$,
	such that 
	$v_1,\ldots,v_p,u_1,\ldots,u_t$ is a $(p+t)$-clique.

	Before the quantum search begins, the nodes list all $p$-cliques in the graph;
	each node $v$ learns all edges in $E(T_1^v,\ldots,T_p^v)$ as described in Section~\ref{sec:TriTri}.

	The setup algorithms $\mathcal{S}_1,\ldots,\mathcal{S}_{t-1}$
	are as follows: in $\mathcal{S}_i$,
	the leader disseminates the current partial search query $(j_1,\ldots,j_i) \in [r_1] \times \ldots \times [r_i]$.
	The network uses Lenzen routing
	so that each $v \in V$ learns the edges
	$E(T_1^v \cup \ldots \cup T_p^v \cup X_1^{j_1} \cup \ldots \cup X_{i-1}^{j_{i-1}}, X_i^{j_i})$.
	The running time $s_i$ of $\mathcal{S}_i$ is
	$O(n^{1-1/p-r_i})$.

	The final classical evaluation procedure, $\mathcal{C}$,
	is as follows: the leader disseminates the query $(j_1,\ldots,j_t) \in [r_1] \times \ldots \times [r_t]$
	to all nodes,
	and the network uses Lenzen routing so that each $v \in V$ learns the edges
	$E(T_1^v \cup \ldots \cup T_p^v \cup X_1^{j_1} \cup \ldots \cup X_{t-1}^{j_{t-1}}, X_t^{j_t})$.
	Together with the edges in $\bigcup_{i < t} \mathsf{setup}_i^t(j_1,\ldots,j_i)$,
	each node $v$ now knows $E(T_1^v,\ldots,T_p^v,X_1^{j_1},\ldots,X_t^{j_t})$.
	Node $v$ now checks whether it sees a $(p+t)$-clique, and informs the leader.
	The running time of $\mathcal{C}$
	is $O(n^{1-1/p-r_t})$.

	The overall running time of the quantum search is given by
	\begin{align*}
		\!\!\!\!\!\!O\!\left( n^{r_1/2} \!\left( n^{1-1/p-r_1} \!+\! n^{r_2/2} \!\cdot \!\left( n^{1-1/p-r_2} \!+\!  \ldots \!+\!  n^{r_{t-1}/2} \left(n^{1-1/p-r_{t-1}} \!+\! n^{r_t/2} \cdot n^{1-1/p-r_t}  \right)\! \right)\!\right) \!\right)\!.
	\end{align*}
	Denote by $g(i)$ the running time of the innermost $t - i + 1$ levels of the search, starting
	from level $i$ up to level $t$:
	\begin{align*}
		g(i) = 
		O\left( n^{r_i/2} \left( n^{1-1/p-r_i} + \ldots +  n^{r_{t-1}/2} \left(n^{1-1/p-r_{t-1}} + n^{r_t/2} \cdot n^{1-1/p-r_t}  \right)  \right) \right).
	\end{align*}
	We claim, by backwards induction on $i$, that
	\begin{equation}
		g(i) = O( n^{(1-1/p)(1 - 1/2^{t-i+1})} ).
		\label{eq:gi}
	\end{equation}
	For the base case, $i = t$, we have 
	\begin{align*}
		g(i)
		&= O\left( n^{r_t/2} \cdot n^{1-1/p-r_t} \right)
		\\
		&= O\left( n^{1-1/p-r_t/2} \right)
		=
		O\left( n^{1-1/p-(1-1/p)^0/2} \right)
		=
		O\left( n^{(1-1/p)/2} \right),
	\end{align*}
	and indeed this matches~\eqref{eq:gi}.
	For the induction step, suppose the claim holds for $i$, and consider $g(i-1)$:
	\begin{align*}
		g(i-1)
		&=
		O\left( n^{r_{i-1}/2} \left( n^{1-1/p-r_{i-1}} + g(i) \right) \right)
		\\
		&=
		O\left( n^{(1-1/p)/2^{t-i+1}/2} \left( n^{1-1/p-(1-1/p)/2^{t-i+1}} + n^{(1-1/p)(1 - 1/2^{t-i+1})} \right) \right)
		\\
		&=
		O\left( n^{(1-1/p)/2^{t-i+2}} \cdot 2n^{(1-1/p)(1 - 1/2^{t-i+1})} \right)
		\\
		&=
		O\left( n^{(1-1/p)(1 - 1/2^{t-i+2})} \right),
	\end{align*}
	again matching~\eqref{eq:gi}.

	The running time of the entire quantum search is
	\begin{equation*}
		g(1) = O\left( n^{(1-1/p)(1 - 1/2^{t})} \right).
	\end{equation*}
\fi



==> app_Congest.tex <==
\section{Missing Proofs from Section~\ref{sec:qcongest}}
\label{app:congest}

\subsection{Missing proofs of Section \ref{subsec:triangles_congest}}
\label{appset_triangles_conget}
\begin{lemma-repeat}{lem:num_of_computation_units}
	In the process described in subsection~\ref{subsec:triangles_congest}, the set of marked computation units is pairwise-independent and is of size at least $\bar{n}/2$.
\end{lemma-repeat}
\begin{proof}
	We note that the set is indeed pairwise independent, as for each node $v$ the edges of the computation units with node $v$ are edge-disjoint.
	
	Recall that $m \leq c\bar{m}$ for some constant $c > 0$. Therefore, the number of edges in $|E\inext|$ is at least $\bar{m}/c$, and the average degree of $G\inext$ is at least $2\bar{m}/(cn\inext) \geq 2\bar{m}/\bar{n} = 2n^\delta$. Assume by contradiction that there are less than $\bar{n}/(2)$ computation units marked. Consider a graph $\tilde{G}$ that is defined by $G\inext$ after removing all edges participating in a marked computation unit. By the assumption there are at most $\bar{n}/(2) \lfloor \bar{n}^\delta/2c \rfloor$ edges removed, meaning that the number of edges in $\tilde{G}$ is at least $\bar{n}^{1+\delta}/(2c)$ edges remaining in $\tilde{G}$. This implies that the average degree in $\tilde{G}$ is at least $\bar{n}^\delta/2c$, meaning that there is at least one node $v$ with degree $\bar{n}^\delta/2c$, which contradicts the process above, as $v$ could have marked an additional computation unit.
\end{proof}

\paragraph{Correctness.}
If the graph is triangle-free then the network accepts, as a computation unit $v$ only rejects if it detects a triangle in the edges $E_1(v) \cup E_2^j(v)$ for some $1 \leq j \leq \bar{n}^{2/5}$. Otherwise, let $\{v_1,v_2,v_3\}$ be vertices of a triangle in $G'$. Let $i,j \in [\bar{n}^{2/5}]$ such that $v_1 \in A_i, v_2 \in A_j$ and let $P_{i,j}$ be the set of computation units that the pair $A_i,A_j$ is mapped to. Let $k \in [\bar{n}^{1/5}]$ and $r \in [\bar{n}^{1/5}]$ such that $v_3 \in S^{(r)}_k$ and let $w \in P_{i,j}$ be the computation unit in $P_{i,j}$ which $S_k$ is mapped to. We note that the triangle is contained in $E_1(w) \cup E^r_2(w)$, and therefore the network rejects in the protocol $A_r$, therefore the global protocol rejects as well. 



%\subsection{Missing proofs from Section \ref{subsec:congestExtend}}
%\label{app:congest:extend}

%\subsubsection{Proof of Theorem \ref{thm:congest:four}}
%\label{app:congest:extend:four}
%
%\begin{theorem-repeat}{thm:congest:four}
%\ThmCongestFour
%\end{theorem-repeat}
%
%To prove the theorem, we first prove the following theorem per cluster.
%
	%Let $G = (V, E)$ be a graph, where $n = |V|$, and let $C = (V_C, E_C)$ be a cluster in an \emph{expander decomposition with high degree clusters (Definition~\ref{def:expanderDecompHighDeg})} of $G$. Denote by $N(C) \subseteq V \setminus V_C$ the set of nodes in $V \setminus V_C$ which have neighbors in $C$, and by $N^{+}(C) = N(C) \cup C$. Let $\bar E \subseteq (V_C \times N(C)) \cap E$, $E_{N(C)} \subseteq (N(C) \times N(C)) \cap E$ be sets of edges. Denote $k = |V_C|$, $q = |E_C|$, $\tilde {n} = |N(C)|$, $\tilde{m} = |E_{N(C)}|$, $\bar m = |\bar E|$, $\mu = q/k$. For any node $v \in N^{+}(C)$, denote by $\deg_{C}(v)$, $\deg_{N(C)}(v)$ the number of neighbors of $v$ in $V_C$, $N(C)$, respectively.
%
%\newcommand{\ThmCongestPfour}
%{
%Let $a$, $b$ be any positive integers such that $a^2b = k$.
%There exists an algorithm in the \qcongest model which detects the existence of an instance of $K_4$ in the graph $G' = (N^{+}(C), E_C \cup \bar E \cup E_{N(C)})$, which contains at least two nodes in $V_C$. The round complexity of the algorithm is $\tilde O((n/b + k/a) / \mu^{1/2} + (n/b + k/a)^{1/2} + a + b + 1)$, w.h.p. The algorithm uses only the edges $E_C \cup \bar E$ for communication. \dtodo{Note that the whp and the tilde are all in terms of $n$}
%}
%
%\begin{theorem}
	%\label{thrm:k4:helper}
%\ThmCongestPfour
%\end{theorem}
%
%\begin{proof}
	%Primarily, as $C$ is a cluster in an \emph{expander decomposition with high degree clusters} (Definition~\ref{def:expanderDecompHighDeg}) of $G$, all of the following hold, by definition. These properties are crucial and widely used throughout the following proof.
	%\begin{enumerate}
		%\item The mixing time of $C$ is $\poly \log(n)$.
		%%\item For every $v \in N(C)$, $\deg_C(v) \geq 1$.
		%\item For every $v \in V_C$, $\deg_{N(C)}(v) = \tilde O(\deg_{C}(v))$. Further implying $\bar m = \tilde O(q)$.
		%\item $\tilde{m}/n \leq m/n = \tilde O(q/k) = \tilde O(\mu)$.
		%% \item For some value $\delta$, it holds that $\mu = \Omega(\delta)$.
	%\end{enumerate}
	%
	%{\bf Triangle Listing.}
	%Create a \emph{randomized} partition of $V_C$ into $a$ parts $V_C^1, \dots, V_C^a$, each of size $\tilde O(k/a)$, w.h.p., and of $N(C)$ into $N^{1}(C), \dots, N^b(C)$, each of size $\tilde O(\tilde{n}/b)$, w.h.p. Specifically, to create the partitions, every node in $v \in N^{+}(C)$ uniformly at random joins one of the parts, denoted $p(v)$, and sends $p(v)$ to all its neighbors in $V_C$, within $1$ round while using only the edges $E_C \cup \bar E$ for communication. Therefore, notice that for every edge $e = \{u, w\} \in E_C \cup \bar E$, both $u$ and $w$ know $p(u)$ and $p(w)$, and therefore we assume that this information is attached to $e$ from here on.
%% \dtodo{fixed -- @keren, this used to be wrong before but now is right}.
	%
	%
%%	\dtodo{elaborated this paragraph}
%Create $k$ \emph{computation units} using the nodes $V_C$. The computational units can be viewed as some \emph{virtual nodes} which can communicate with one another and are simulated by $V_C$. Precisely, every node $v \in V_C$ with $\deg_C(v) = \Omega(\mu)$ creates $\Theta(\deg_C(v)/\mu)$ computational units which it simulates. Each computation unit can send and receive $\mu$ messages to and from any other computational unit in the cluster within $O(1)$ rounds. Observe that, by choosing appropriate constants, it can be ensured that there are exactly $k$ computational units simulated in $V_C$, as $\sum_{v \in V_C} \Theta(\deg_C(v)/\mu) = \Theta(q / \mu) = \Theta(k)$. Due to Claim~\ref{claim:2approx}, within $\poly \log (n)$ rounds, every node in $V_C$ can compute a $2$-approximation to the degree of every other node in $V_C$, and thus all the nodes in $V_C$ can know how many computational units are simulated at each node and which node simulates which units.
	
%	\dtodo{editted a bit}
%Every computational unit is assigned exactly one triad (out of a total of $k$ triads) composed of two sets in the partition of $V_C$ and one set in the partition of $N(C)$. Let $v \in V_C$ be a node with at least one computational unit, and observe a single computational unit which is assigned to $v$, denoted $c_v$.  Denote by $V_C^i$, $V_C^j$ and $N^\ell (C)$ the sets corresponding to $c_v$, for some indices $i,j$ and $\ell$. The assignment of the sets to the computational units is hardcoded and is thus globally known. From here on and until the end of the proof, we continue with these specific $v$, $c_v$, $V_C^i$, $V_C^j$ and $N^\ell (C)$.
	
	%Further, as the partitions are independent, we get that w.h.p., $|E(V_C^i, V_C^j)| = \tilde O(|E_C|/a^2 + 1) = \tilde O(q/a^2 + 1) = \tilde O(\mu k / a^2 + 1) = \tilde O(\mu b + 1)$, and, $|E(V_C^j, N^\ell (C))| = \tilde O(|\bar E|/(a\cdot b) + 1) = \tilde O(\bar m / (a \cdot b) + 1) = \tilde O(q / (a \cdot b) + 1) = \tilde O(\mu k / (a \cdot b) + 1) = \tilde O(\mu a + 1)$ (likewise with $|E(N^\ell (C), V_C^i)|$).
%\ktodo{please explain how we get these}\dtodo{fixed a small mistake and elaborated}.
	
	%\dtodo{elaborated on all the paragraph -- it is possible to slightly shorten the text here using Claim~\ref{claim:batchMessaging}, however, this is already written and so we might not want to touch it} 
	%Thus, the unit $c_v$ can learn the edges $E(V_C^i, V_C^j)$, $E(V_C^j, N^\ell (C))$ and $E(N^\ell (C), V_C^i)$, within $\tilde O(a + b + 1)$ rounds, w.h.p., using only the $\mu$ bandwidth allocated by $v$ to $c_v$. To see this, notice that every edge which $c_v$ needs to learn is known to some node in $V_C$. Observe that the assignment of the sets to $c_v$ is known, the assignment of $c_v$ to $v$ is known, and for every edge in $e = \{u, w\} \in E \cup \bar E$, both $u$ and $w$ know to which sets $u$ and $w$ belong to. Thus, if $u \in V_C$ is incident to an edge $e$ which $c_v$ needs to learn, then $u$ knows to send $e$ edge to $v$. We showed that $c_v$ needs to receive at most $\tilde O(\mu a + \mu b + 1)$ messages. We now show that every $v$ needs to send at most $\tilde O(\deg_C(v) \cdot (a + b))$ messages. To see this, denote by $V_C^{\alpha(v)}$ the part such that $v \in V_C^{\alpha(v)}$, and let $e = \{v, w\} \in E_C$ and $e = \{v, u\} \in \bar E$ be edges incident to $v$, with the corresponding nodes $w \in V_C^{\alpha(w)}$ and $u \in N^{\beta(u)}(C)$. Notice that there are exactly $b$ computation units which are assigned both $V_C^{\alpha(v)}$ and $V_C^{\alpha(w)}$, implying that $e$ needs to be sent by $v$ to at most $b$ nodes. Similarly, exactly $a$ computational units are assigned both $V_C^{\alpha(v)}$ and $N^{\beta(u)}(C)$. Thus, in total, $v$ needs to send at most $O(\deg_C (v) \cdot b + \deg_{N(C)}(v) \cdot a) = \tilde O(\deg_C(v) \cdot (a+b))$ messages. Having shown the above constraints on how many messages each node sends and receives, by Theorem~\ref{thm-expander-routing}, this routing can be accomplished in $\tilde O(a + b + 1)$ rounds, w.h.p., as claimed.
	
	%Notice that the algorithm up to this stage lists all $K_3$ involving at least two nodes in $V_C$, within $\tilde O(a + b + 1)$ rounds.\vspace{2mm}
	
%\noindent{\bf Quantum Searches.}
	%Create a degree-based partition of $N^{+}(C)$. Every node $u \in N^{+}(C)$ computes $f(u) = \deg_C(u)/a$, $g(u) = \deg_{N(C)}(u)/b$ \dtodo{address what happens when this is smaller than $1$}. Notice that $f(u)$ is an upper bound on the expected number of neighbors $u$ has in $V_C^i$, likewise in $V_C^j$, and $g(u)$ is a similar upper bound w.r.t. $N^\ell (C)$.  Finally, $u$ computes the value $h(u) = f(u) + g(u)$. It always holds that $h(u) \leq k/a + \tilde{n}/b \leq k / a + n / b$, it is possible to partition $N^{+}(C)$ into  $A_1, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ whereby $u \in A_{\lfloor \log (h(u)) \rfloor}$.
	%
	%Observe that $h(N^{+}(C)) = \sum_{u \in N^{+}(C)} h(u) = \sum_{u \in N^{+}(C)} \deg_C(u)/a + \deg_{N(C)}(u)/b = O((m + \bar m) / a + (\tilde{m} + \bar m) / b) = \tilde O(q / a + (\mu n + q) / b) = \tilde O(\mu k / a + ( \mu n + \mu k ) / b) = \tilde O(\mu k / a + \mu n /b)$, where the last transition is due to the fact that $k \leq n$, and the rest of the transitions follow from the properties of $C$ stated at the start of this proof.
	%
	%We iterate over all the sets $A_1, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ sequentially. Due to the fact that we desire to utilize the available bandwidth as much as possible, we treat nodes with low $h(\cdot)$ by coalescing them together, while those with high $h(\cdot)$ are dealt with in a different manner. As such, we have two different algorithms, for \emph{low-cost} and \emph{high-cost} nodes.\vspace{2mm}
	
%\noindent{\bf Low-Cost Nodes.}
%Iterate over the sets $A_1, \dots A_{\lfloor \log \mu \rfloor}$ sequentially. From here on, fix $\tau \in [\lfloor \log \mu \rfloor]$, and observe $A_\tau$.
	
	%Construct an arbitrary BFS tree over $V_C \cup A_\tau$, which completes in $\poly \log (n)$ rounds, as the mixing time of $C$, and hence the diameter of $V_C \cup A_\tau$, is at most $\poly \log (n)$. Use this tree to number the nodes in $A_\tau$ from $1$ to $|A_\tau|$, and so, from now on, w.l.o.g., assume that the identifiers of the nodes in $A_\tau$ are in $[|A_\tau|]$.
	
	%By definition, every node $v \in A_\tau$ satisfies $2^{\tau-1} < h(v) \leq 2^\tau$. Further, recall that $h(A_\tau) \leq h(N^{+}(C)) = \tilde O(\mu k / a + \mu n/b)$. Therefore, it is possible to create a partition of $A_\tau$ into $A_\tau^1, \dots, A_\tau^{k / a + n/b}$, whereby for every $\gamma \in [k / a + n/b]$, it holds that $h(A_\tau^j) = O(\mu + 2^\tau) = O(\mu)$, where the last transition holds as $\tau \leq \log \mu$. %\ktodo{Square brackets and $\{..\}$ in the calculations, what do they mean? Can they be replaces with the standard?}\dtodo{They do not mean anything special -- can be replaced. Will go over and replace when we have some downtime}
	
	%\dtodo{elaborated} 
	%Perform a Grover search over $\gamma \in [k / a + n/b]$ to check whether an instance of $K_4$ exists which has at least two nodes in $V_C$ and involves at least one node from $A_\tau^\gamma$. Recall node $v \in C$ denoted above, along with $c_v$, $V_C^i$, $V_C^j$ and $N^\ell (C)$ . In order for $c_v$ to check if any $K_3$ which it sees using the edges between $V_C^i$, $V_C^j$ and $N^\ell (C)$ can be extended to a $K_4$ using a node from $A_\tau^\gamma$, it suffices for $c_v$ to learn the edges between all the nodes in $A_\tau^\gamma$ and each of these three sets. Denote by $\rho(i, j, \ell, \gamma)$ the number of such edges. Notice that $h(A_\tau^\gamma) = \tilde O(\mu)$ upper bounds the expectation of $\rho(i, j, \ell, \gamma)$. Thus, w.h.p., $c_v$ needs to receive $\tilde O(\rho(i, j, \ell, \gamma) + 1) = \tilde O(\mu + 1) = \tilde O(\mu)$ messages. Therefore, in total, $\tilde O(k \cdot \mu ) = \tilde O(q)$ messages need to be delivered, as there are $k$ computational units.
	
	%
	%\dtodo{begin remove} On the contrary, we need to show that $v$ sends at most $\tilde O(\deg_C(v) + 1)$ messages. \dtodo{complete routing}
	
	%Having shown the above constraints on how many messages each node sends and receives, using Theorem~\ref{thm-expander-routing} this routing can be accomplished in $\tilde O(1)$ rounds, w.h.p. \dtodo{end remove}
	%
	%As the Grover search is over $\gamma \in [k / a + n/b]$, and checking for each $\gamma$ requires $\tilde O(1)$ rounds, w.h.p., the search can be performed in $\tilde O((k / a + n/b)^{1/2})$ rounds, w.h.p., using Lemma~\ref{lemma:qsearchv0}.\footnote{Notice that Lemma~\ref{lemma:qsearchv0} requires a \emph{leader} for the Grover search, however, as the diameter of $C$ is $\poly \log (n)$, this leader can be any arbitrary node within $C$, implying a round complexity cost which is multiplicative in $\poly \log (n)$.}\vspace{2mm}
	%
%\noindent{\bf High-Cost Nodes.} Iterate over the sets $A_{\lfloor \log \mu \rfloor + 1}, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ sequentially. Fix $\tau \in [\lceil \log (k / a + n / b) \rceil] \setminus [\lfloor \log \mu \rfloor]$, and observe $A_\tau$.
	%
    %The current goal is to check for the existence of an instance of $K_4$ which contains at least two nodes in $V_C$ and one node in $A_\tau$.  Perform a Grover search over $w \in A_\tau$.
	% Recall node $v \in C$ denoted above, with its specific computational unit and the corresponding sets $V_C^i$, $V_C^j$ and $V_{\partial C}^\ell$ . In order for $v$ to check if any $K_3$ which it sees using the edges between $V_C^i$, $V_C^j$ and $V_{\partial C}^\ell$ can be extended to a $K_4$ using $w$, it suffices for $v$ to learn the edges between $w$ and each of these three sets.
	
	%\dtodo{elaborated} 
	%Similarly to the \emph{Low-Cost} case, $c_v$ needs to learn the edges between $w$ and all the nodes in $V_C^i$, $V_C^j$ and $N^\ell (C)$. Denote by $\rho'(i, j, \ell, w)$ the number of such edges. Notice that $h(w) = O(2^\tau)$ upper bounds the expectation of $\rho'(i, j, \ell, w)$. Thus, w.h.p., $c_v$ needs to receive $\tilde O(2^\tau + 1)$ messages. Therefore, in total, $\tilde O(k \cdot (2^\tau + 1) )$ messages need to be delivered, as there are $k$ computational units.

	%\dtodo{added this} 
	%On the contrary, for every edge $e = \{w, u\}$ incident to $w$, node $u$ sends $e$ to some node in $C$ which neighbors $u$. Observe now that all the edges incident to $w$ are known to the nodes of $C$. Given $e$, it is possible to compute all of the computational units which require $e$ if one knows the part in the partition to which $u$ belongs. This information is available, as $u$ can just attach the number of its part to $e$. Further, every node $x \in V_C$ receives at most $\deg(x) = \deg_C(x) + \deg_{N_C}(x) = \tilde O(\deg_C(x))$ such edges to be responsible for. As such, recalling that in total $\tilde O(k \cdot (2^\tau + 1) )$ messages need to be delivered, one can use the \emph{batch-messaging} algorithm from Claim~\ref{claim:batchMessaging} in order to deliver these messages within $\tilde O(k \cdot (2^\tau + 1) / q ) = \tilde O(2^\tau / \mu + 1) = \tilde O(2^\tau / \mu)$ rounds, w.h.p., where the last transition follows since $2^\tau = \Omega(\mu)$.
	
	 %\dtodo{explain the routing involved. First, node $w$ sends its edges into the cluster by having each of its nodes outside the cluster say that they neighbor $w$ to someone in the cluster -- this takes $O(1)$ rounds. Then, we can arbitrarily reshuffle the edges inside the cluster in order to be able to send them nicely. Perhaps have a general reshuffling theorem which can also be used above when we do the triangle listing stage}.
	
	 %Having shown the above constraints on how many messages each node sends and receives, using Theorem~\ref{thm-expander-routing} this routing can be accomplished in $O(2^\tau / \mu)$ rounds, w.h.p.
	
	%As $h(N^{+}(C)) = \tilde O(\mu k / a + \mu n/b)$, we get that $|A_\tau| = \tilde O((\mu k / a + \mu n / b)/2^\tau)$. Thus, the Grover search takes $\tilde O(((\mu k / a + \mu n / b)/2^\tau)^{1/2} \cdot 2^\tau / \mu) = \tilde O((k / a + n / b)^{1/2} \cdot (2^\tau / \mu)^{1/2})$ rounds, w.h.p., using Lemma~\ref{lemma:qsearchv0}. As $2^\tau = O(n/b + k/a)$, we get a final complexity of $\tilde O((k / a + n / b)^{1/2} \cdot ((n/b + k/a) / \mu)^{1/2}) = \tilde  O((n/b + k/a) / \mu^{1/2})$.
%\end{proof}
%
%
%Using the above, we can now show the following main result. That is, given a specific cluster $C$, with corresponding $k$ and $\mu$, the following algorithm chooses the optimal $a$ and $b$ positive integers in order to execute the previous claim with.
%\begin{theorem-repeat}{thm:congest:four}
%\ThmCongestFour
%\end{theorem-repeat}
%
%\begin{proof}
	%Primarily, we invoke the diameter reduction procedure described in Lemma~\ref{thm:diameter_reduce},which allows us to assume w.l.o.g. that $D$, the diameter of $G$, is at most $\poly \log (n)$.
	%
	%We proceed recursively,
	%%apply the expander decomposition detailed in Lemma~\ref{lemma:decomp},
	%and in each iteration we remove a constant factor of either the nodes or the edges, implying that we halt after at most $\poly \log (n)$ iterations.
	%
	%Perform the following algorithm for at most $\poly \log (n)$ iterations. First, compute the average degree of the graph, that is $\mu_G = \Theta(|E|/|V|)$, taking at most $O(D) = \poly \log (n)$ rounds.
	%If $\mu_G \leq n^{4/9}$, then every node with degree at most $2n^{4/9}$ learns its induced 2-hop neighborhood, using Claim~\ref{claim:2hopNeighborhood}, in $O(n^{4/9})$ rounds, lists all the cliques it sees involving itself, and exits. In the case that this happens, it is ensured that at least half of the nodes in the graph exit at this iteration \dtodo{ref}.
	%Otherwise, that is, if $\mu_G > n^{4/9}$, invoke the expander decomposition detailed in Lemma~\ref{lemma:decomp}. As $\mu_G > n^{4/9}$, by Lemma~\ref{lemma:decomp} it holds that for every   %and receive clusters which satisfy all of the properties required in Theorem~\ref{thrm:k4:helper} \dtodo{potentially extract to a definition}, with the additional constraint that for every
	%cluster $C$ in the decomposition, the average degree in the cluster, $\mu_C$ satisfies $\mu_C = \Omega(n^{4/9})$.
	%
	%In the case that we run the expander decomposition, we proceed to detecting a $K_4$ which contains at least one edge inside one the clusters, if there exists such. Once we do this, it is possible to remove all the cluster edges from the graph, as removing them cannot remove an edge from any $K_4$ which was not already checked for. As the expander decomposition guarantees that at least a constant fraction of the edges are in the clusters, we can conclude the iteration.
	%
	%Therefore, we need to show how every cluster can detect a instance of $K_4$ which contains at least one edge inside the cluster, if there exists such. We run the following algorithm for each cluster. Observe that the algorithm only uses the edges inside the cluster as well as the edges crossing the cluster boundary (have exactly one endpoint in the cluster) for communication. This implies that all the clusters can execute the algorithm in parallel -- edges internal to a cluster are only used by it, and every edge between clusters is only used by two clusters, implying that we at most double the round complexity of the algorithm if all clusters run in parallel (i.e. we can assume w.l.o.g. that every cross-cluster edge sends on even round messages from the high end point to the low, and vice versa during odd rounds).
	%
	%\dtodo{Try to play around with the numbers here, to see if we can get any better (see comment here): %https://www.wolframalpha.com/input/?i=minimize+max%281-b-x%2F2%2C+1-a-x%2F2%2C+a%2C+b%2C+x%29+where+2a%2Bb+%3D+1%2C+a+%3E%3D+0%2C+b+%3E%3D+0%2C+x+%3E%3D+0%2C+k%3D1%2C+w.r.t.+a%2C+b%2C+x
	%Note: It currently seems that $k=0.8$ is the big problem. If we assume $k\geq 0.9$, we get $21/45$ round complexity, and if we assume $k = 1$ we get $20/45$. For smaller $k$, we should let $a$ be bigger instead of setting $a = b$.
	%}
	
	%Observe a specific cluster $C = (V_C, E_C)$ which we computed in the decomposition. Our goal is to detect any instance of $K_4$ in $G$ which contains at least two nodes in $V_C$. We break into cases depending on $k = |V_C|$.
	
	%If $k = \tilde O(n^{2/5})$, then every node $v \in V_C$ learns its induced 2-hop neighborhood in $\tilde O(n^{2/5})$ rounds, using Claim~\ref{claim:2hopNeighborhood}.
	
	%If $k = \omega(n^{2/5})$ and $k = \tilde O(n^{4/5})$, then set $b = n^{2/5}$, $a = k^{1/2}/n^{1/5}$. Observe that $a^2 b = k$, and that $a = k^{1/2}/n^{1/5} =  \omega(n^{1/5}/n^{1/5}) = \omega(1)$, implying that we can assume $a$ is an integer, as rounding it would not change its value by more than a constant factor. Therefore, we can execute Theorem~\ref{thrm:k4:helper} within $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b)$ rounds, w.h.p., where $\mu_C = \Theta(|E_C|/|V_C|)$. As stated above, due to the parameters we used, it is ensured that $\mu_C = \Omega(n^{4/9})$, and thus the total round complexity is $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b) = \tilde O((n^{3/5} + k^{1/2}n^{1/5})/n^{2/9} + (n^{3/5} + k^{1/2}n^{1/5})^{1/2} + k^{1/2}/n^{1/5} + n^{2/5}) = \tilde{O} (n^{3/5}/n^{2/9} + n^{3/10} + n^{1/5} + n^{2/5}) = \tilde O(n^{17/45})$, w.h.p., which is bounded by $\tilde O(n^{4/9})$.
	
	%Finally, $k = \omega(n^{4/5})$ and $k \leq n = \tilde O(n)$. We set $b = n^{1/3}$, and $a = k^{1/2}/n^{1/6}$. Notice that $a^2 \cdot b = k$, and that $a = k^{1/2}/n^{1/6} =  \omega(n^{2/5}/n^{1/6}) = \omega(n^{7/30}) = \omega(1)$, implying that we can assume $a$ is an integer. Recall that $\mu_C = \tilde \Omega(n^{4/9})$. The total round complexity is thus $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b) = \tilde O((n^{2/3} + k^{1/2}\cdot n^{1/6}) / n^{2/9} + (n^{2/3} + k^{1/2}\cdot n^{1/6})^{1/2} + n^{1/3} + k^{1/2}/n^{1/6}) = \tilde O(n^{4/9} + n^{1/3} + n^{1/3}) = \tilde O(n^{4/9})$, w.h.p.
%\end{proof}

%\begin{comment}
%\dtodo{DEPRECATED FROM HERE ON}
%\dtodo{Sketch}

%Given values $\delta$, $\kappa$, define the following algorithm. After we compute the expander decomposition (Step 2d in the algorithm), the algorithm works on a cluster-basis manner, and we denote the given cluster by $C$. Denote by $\partial C$ the nodes incident to $C$ -- that is, nodes which themselves are not in $C$, yet have neighbors in $C$. The algorithm only uses for communication the edges in $E(C, C)$ and $E(C, \partial C)$. For any node $v \in C \cup \partial C$, denote by $deg_C(v)$, $deg_{\partial C}(v)$ and $deg (v)$ the number of neighbors $v$ has in $C$, in $\partial C$, and in total, respectively. Note that it does not have to hold that the sum of the first two equals the third, as $C \cup \partial C$ does not necessarily cover all the nodes in the graph, however, for simplicity, we treat it as if the inequality does indeed hold.
%
%\dtodo{Note: Unlike what we currently do with the algorithm in the SODA paper, here, we actually change the listing algorithm (for $K_3$) and make it run a bit slower. This overall makes us faster in terms of detection (for $K_4$) -- it is necessary in order to break below $o(n^{1/2})$.}
%
%\begin{enumerate}
	%\item For simplicity, execute the diameter reduction algorithm that Orr and Rotem mentioned to w.l.o.g. assume $D = \poly \log (n)$.
	%\item While the graph is not empty:
	%\begin{enumerate}
		%\item Compute $\mu$, the average degree of the graph, in $O(D) = \poly \log (n)$ rounds.
		%\item If $\mu \leq \delta$, then:
		%\begin{enumerate}
			%\item Any node $v$ where $deg (v) \leq 2 \delta$ learns its 2-hop neighborhood in $O(\delta)$ rounds, lists all the cliques which include itself, and removes itself and its incident edges from the graph.
			%\item Go back to the beginning of the while loop. Analysis: in the step above, at least half of the nodes were removed from the graph, implying that we will reach this stage (and jump back to the start of the while loop) at most $\log n$ times.
		%\end{enumerate}
		%\item From here on, we can assume $\mu > \delta$.
		%\item Compute an expander decomposition in $\poly \log n$ rounds. We now proceed to describe the algorithm for each cluster $C$.
		%\item Denote $k = |C|$. If $k \leq \kappa$, every node in $C$ learns its 2-hop neighborhood in $\tilde O(\kappa)$ rounds (as the CS decomposition guarantees that for $v \in C$, it holds that $deg_{\partial C}(v) = \tilde O(deg_C(v))$), lists all the cliques involving itself, and the cluster is removed from the graph.
		%\item Denote by $\mu_C$ and $\mu_{\partial C}$ the average degree of the nodes in $C$ and $\partial C$, respectively. If $\mu_C = o(\mu_{\partial C})$, or, if $\mu_C = o(\delta)$, then $C$ does nothing during the current iteration of the while loop. Using the proof of Claim 4.4 in SODA, plus the fact that $\mu > \delta$, it is possible to show that this step causes at most a constant fraction of the edges of the graph to be delayed to the next iteration. \dtodo{Note: In CPZ, they also remove nodes $v \in C$ from $C$ which are such that $deg_C(v) < deg_{\partial C}(v)$ -- this isn't necessary anymore since the CS decomposition guarantees that for $v \in C$, it holds that $deg_{\partial C}(v) = \tilde O(deg_C(v))$, which is good enough.}
		%\item Let $a$, $b$ be two values which we define later. Split $C$ into $C_1, \dots, C_a$ uniformly at random, where $|C_i| = \tilde O(k /a)$ w.h.p.. Split $\partial C$ into $\partial C_1, \dots, \partial C_b$, where $|\partial C_i| = \tilde O(|\partial C|/b) = \tilde O(n/b)$. \dtodo{Notice that in the CPZ alg, $a = b = k^{1/3}$. We have to choose the values differently so that our detection algorithm will be faster.}
		%\item We define $a^2b$ triads -- $C_i$, $C_j$, $\partial C_\ell$, where $i, j \in [a]$, $\ell \in [b]$. We later ensure that $a^2b = k$. Let $v \in C$. We assign to $v$ a number of triads which is $\Theta(deg_C(v)/\mu_C)$. Basically, this means that for every $\mu_C$ bandwidth (up to a constant) which $v$ has, it is assigned one triad. \dtodo{Orr gave this the notation of ``computational units''.} Therefore, from now on we will analyze how a single triad is dealt with using $\mu_C$ bandwidth, in order to let us ignore what happens at every specific node. Notice that every triad is assigned to one node in $C$, and that the assignment of triads to nodes in $C$ can be computed locally by every node in $C$ using tricks shown in CPZ.
		%\item Let node $v$ be responsible for triad $C_i$, $C_j$, $\partial C_\ell$. It is possible that $v$ is responsible also for other triads, however, we assume that $v$ only allocates $\mu_C$ of its bandwidth in every round to dealing with this specific triad. Node $v$ learns the edges between the sets. This takes $O(\mu_C k / (\mu_C a^2)) = O(b)$ rounds to learn the edges between $C_i$ and $C_j$, and $\tilde O(\mu_C k / (\mu_C ab)) = \tilde O(a)$ rounds (since the number of edges crossing the boundary of $C$ is roughly at most the number of edges inside $C$, due to the cluster decomposition) to learn the edges between $\partial C_\ell$ and each of $C_i$, $C_j$. All in all, this step takes $O(a + b)$ rounds.
		%\item Cluster $C$ splits the nodes in $\partial C$ into sets $\partial C^1, \dots \partial C^{\log n}$ \dtodo{In the part where we analyze the SODA algorithm, we use $\partial C_i$ for this notation, so change this part to match}, where $v \in \partial C^{i}$ if its degree is between $2^{i-1}$ and $2^i$. For each $i \in [\log n]$, do the following.
		%\begin{enumerate}
			%\item Grover search over node $w \in \partial C^i$. This takes $|\partial C^i|^{1/2}$ iterations of the following algorithm. Notice that $|\partial C^i| \cdot 2^i = O(\mu_C \cdot n)$, implying $|\partial C^i| = O(\mu_C \cdot n / 2^i)$.
			%\begin{enumerate}
				%\item We wish to see if it is possible to extend a $K_3$ which has been listed by $C$ to a $K_4$ using $w$.  \dtodo{We assume here that $w \in \partial C$, we also need to check for $w \in C$, but that should not be a problem}. To do so, we need to send the edges incident to $w$ to the nodes in $C$ which need them. To do so, we show one algorithm to send between $w$ and other nodes in $\partial C$, and one which deals with the edges between $w$ and nodes in $C$.
				%\item First, the cluster broadcasts to $C \cup \partial C$ that we are searching over node $w$ now \dtodo{how does anyone know who $w$ is? Should be solvable, e.g. by $w$ choosing with some probability if it wants to go in this iteration, or something similar}. Then, every node which neighbors $w$ tells some node in $C$ about the edge between it and $w$. Thus, now all the edges in $E(\{w\}, C \cup \partial C)$ are known to nodes in $C$ \dtodo{need to reshuffle the edges so that each node in $C$ holds a number of edges proportional to its degree, etc -- arbitrary reshuffle is ok since the degree of a node from $C$ to other nodes in $C$ is at least roughly that as the number of neighbors it has in $\partial C$.}
				%\item Let there be a specific triad $C_d$, $C_e$, $\partial C_f$, and $v$ the node responsible for the triad. W.h.p., $w$ neighbors $|\partial C_f| \cdot 2^i / |\partial C| = 2^i / b$ nodes in $\partial C_f$, requiring $\tilde O(2^i / (b \mu_C))$ rounds to deliver these edges to $v$ \dtodo{again, need some load balancing in terms of who sends which messages, but this is doable}. \dtodo{Total runtime that we get: $\tilde O(2^i / (b \mu_C))$ per iteration, and we have $O(\sqrt{\mu_C \cdot n / 2^i})$ iterations due to Grover. The product comes out to at most $O(n/(b \sqrt{\mu_C}))$ rounds.}
				%\item \dtodo{Need to deal with the edges between $w$ and $C$ -- need to send them as well -- might require two different algorithms dependent on $k$....} \dtodo{We also have a small bug: for low $i$, we need to coalesce some nodes together when searching so that we don't waste bandwidth -- should not be a problem.}
			%\end{enumerate}
		%\item  \dtodo{In the end, we set $\kappa = \delta = b = n^{2/5}$, and this is also the round complexity which we get}
		%\end{enumerate}
%
		%
	%\end{enumerate}
%\end{enumerate}

%
%\end{comment}


%%%
%%% p=7
%%%

\subsection{Proof of Theorem \ref{theorem:K6detectQcongest}}
\label{app:congest:extend:seven}

\begin{theorem-repeat}{theorem:K6detectQcongest}
\ThmCongestPseven
\end{theorem-repeat}

\begin{proof}
We begin by briefly explaining the $K_p$ listing algorithm of \cite{Censor+SODA21}. The algorithm of \cite{Censor+SODA21} works in iterations, which are composed of stages. In every stage, some $K_p$ in the graph may be listed.  We split the listed $K_p$ instances according to the stage in the algorithm in which they are listed. For each stage, we show how to detect in a quantum manner if there is an instance of $K_p$ that is listed in that stage which can be extended to (i.e., is a part of) an instance of $K_{p+1}$. As such, if there is any instance of $K_{p+1}$ in the graph, then we will certainly detect this as some instance of $K_p$ could be extended to it.

We now show the $K_p$ algorithm, and interject at appropriate places in order to perform quantum searches. Each iteration of the algorithm of \cite{Censor+SODA21} consists of the following steps.\vspace{2mm}
		
		\noindent{\bf Exhaustive search detection stage.} Every node $v$ with degree $O(n^{1/2})$ learns its induced 2-hop neighborhood in $O(n^{1/2})$ rounds using Claim~\ref{claim:2hopNeighborhood}, lists any cliques which it sees involving itself, and removes itself, along with its incident edges from the graph.
		
		\textbf{Detection of \boldmath{$K_{p+1}$}:} In particular, because the entire induced 2-hop neighborhood is learned, any instance of $K_{p}$ that is listed that can be extended to an instance of $K_{p+1}$ can be immediately listed in this way even without further communication, which proves our claim for this stage.\vspace{2mm}
		
		\noindent{\bf Graph decomposition and cluster exhaustive search detection stage.} An expander decomposition is computed according to Lemma~\ref{lemma:decomp}, while the above ensures that the average degree in the graph (and thus in the clusters, due to Lemma~\ref{lemma:decomp}) is at least $\Omega(n^{1/2})$. In clusters with $O(n^{1-2/p})$ nodes, each node learns its induced 2-hop neighborhood in $G$ using Claim~\ref{claim:2hopNeighborhood} and lists all the instances of $K_p$ which it is a part of, and finally removes itself and its incident edges from the graph. Because Lemma~\ref{lemma:decomp} promises that the number of edges that leave $C$ is at most $\tilde{O}(E_C)$, where $E_C$ are the edges inside $C$, and then this completes in $O(n^{1-2/p})$ rounds.
		
		\textbf{Detection of \boldmath{$K_{p+1}$}:}  As in the previous stage, because of the exhaustive search nature of this stage, we again obtain that any instance of $K_{p}$ that is listed that can be extended to an instance of $K_{p+1}$ can be immediately listed in this way even without further communication, which proves our claim for this stage.\vspace{2mm}
		
					
		\noindent{\bf Cluster listing.} Within every remaining cluster $C$, some nodes are designated as \emph{good} and the rest as \emph{bad}. Let $v$ be a good node. The nodes of $C$ learn amongst themselves all the edges in the induced 2-hop neighborhood of $v$. That is, the nodes of $C$ request from the nodes neighboring the cluster to send in edges from outside $C$ to nodes inside $C$, such that all the induced 2-hop neighborhood of $v$ is known to the nodes in $C$. Now, the nodes in $C$ ensure that every instance of $K_p$ involving $v$ and at least one other node in $C$ is becomes known to some node in $C$ -- that is, these $K_p$ instances are listed by $C$. The good nodes are then removed from the graph along with all of their edges. \vspace{3mm}

\noindent This concludes the description of the \congest algorithm in~\cite{Censor+SODA21}. The exact definition of good nodes is not required for our purpose.
%Also, we mention that during this stage, clusters whose average inner-degree is too small compared to average outer-degree of nodes neighboring the cluster are ignored and their edges are deferred to future iterations.
The proof of \cite{Censor+SODA21} shows that each iteration completes within $\tilde{O}(n^{1-2/p})$ rounds, and that after $\poly \log (n)$ iterations the remaining graph is empty and hence $\tilde{O}(n^{1-2/p})$ rounds are sufficient for the entire algorithm.\vspace{3mm}

		\noindent{\bf The cluster quantum detection stage.}
		We now provide the quantum procedure that we run after the above \textbf{Cluster listing} stage, in order to detect an instance of $K_{p+1}$ that contains an instance of $K_p$ that was listed during this stage. First, let the $C$-degree of a node be its number of neighbors in $C$,
%		recall that $n^{\delta} = n^{1/2}$ is a lower bound on
let $\mu_{C}$ be
		the average $C$-degree of nodes in $C$, and let $H(C)$ be the high $C$-degree cluster nodes, namely, those of $C$-degree $
		%\Omega(n^{\delta}) = \Omega(n^{1/2})$.
\Omega(\mu_{C})$.  Notice that due to the invocation above of Lemma~\ref{lemma:decomp}, it holds that $\mu_C = \Omega(n^{1/2})$.
		A more precise description of the algorithm in~\cite{Censor+SODA21} is that the induced 2-hop neighborhood of each good node $v$ becomes known to the nodes in $H(C)$ rather than to any node in $C$. Second, denote by $N^{+}(C)$ the set of nodes which have a neighbor in $C$ (this includes all of $C$ as $C$ is connected, by definition) and by $N(C) = N^{+}(C)-C$ the neighbors of $C$ outside of $C$. In the above \textbf{Cluster listing} stage we piggyback the degree (not $C$-degree) of every node in $N(C)$ onto the messages containing its edges, so that the degrees of all nodes in $N(C)$ are also known to nodes of $H(C)$.
		
The quantum process starts with the following. The nodes in $C$ elect some arbitrary leader $v_C \in H(C)$.
%and construct a virtual binary tree $T_C$ rooted at $v_C$ which spans $H(C)$, and has depth at most $\poly \log (n)$.
This can be done in $\poly \log (n)$ rounds because this is a bound on the diameter of the cluster, by Lemma~\ref{lemma:decomp}. The nodes of $H(C)$ now broadcast within $H(C)$ the degrees of all the nodes in $N(C)$. This is done in two steps. In the first step, each node in $H(C)$ sends $v_C$ the degrees of nodes in $N(C)$ which it knows about.
%Then, every node tells $v_C$ about the degrees of nodes in $N(C)$ which it knows about.
As every node sends and receives at most $|N(C)| = O(n)$ pieces of information, and every node in $H(C)$ has $C$-degree at least $\Omega(\mu_C) = \Omega(n^{1/2})$, this takes at most $\tilde O(n^{1/2})$ rounds, using the routing algorithm of Theorem \ref{thm-expander-routing}. In the second step, $v_C$ makes this information known to all nodes in $H(C)$ using a simple doubling procedure: in each phase of this procedure, each informed node shares the information with a unique uninformed node. Each phase completes in $\tilde O(n^{1/2})$ rounds by the same argument using the routing algorithm of Theorem~\ref{thm-expander-routing}, and the number of phases is logarithmic. In a similar fashion, the nodes in $H(C)$ learn all the degrees of the nodes in $C$.
%Finally, the information is broadcast to all of $H(C)$ over $T_C$ \ktodo{Do we actually need to reference the SPAA21 paper? This looks trivial to me.}. In a similar manner, the nodes of $H(C)$ also broadcast amongst themselves the $C$-degrees of all nodes in $C$. \dtodo{This seems like some stuff is repeated in the paragraph multiple times.}

Knowing the degrees of all nodes in $N^{+}(C)$, the nodes $H(C)$ \emph{bucket} $N^{+}(C)$ by degrees. That is, they compute $N^{+}(C) = N^{+}_1(C), \dots, N^{+}_{\log n}(C)$, such that the degree of any $v \in N^{+}_i(C)$ is in $[2^{i-1},\dots,2^i)$. We iterate over the $\log n$ buckets, whereby in each bucket we check whether a node in $N^{+}_i(C)$ can be used to extend some $K_p$ instance, which is already listed by $H(C)$, into an instance of $K_{p+1}$. This is done as follows.

Fix an $i$ between 1 and $\log n$. We perform a Grover search over $v \in N^{+}_i(C)$ using $v_C$ as the leader of the search: In each query (i.e., over such a $v$), we broadcast within $H(C)$ all the neighbors of $v$ which are known to $H(C)$, in order to try to extend any $K_p$ listed by $H(C)$ to a $K_{p+1}$ involving $v$. Let $\kappa_{p}$ be such a $K_p$. As it is listed by $H(C)$, it must involve at least one good node in $C$, denoted $g \in \kappa_{p}$. Further, recall that every edge in the induced 2-hop neighborhood of $g$ is known to $H(C)$. Thus, if $v$ that can be used to extend $\kappa_{p}$ to an instance of $K_{p+1}$, all the edges between $v$ and $\kappa_{p}$ are known to the nodes of $H(C)$. Therefore, if we manage to broadcast in $H(C)$ all the edges incident to $v$ that are known to $H(C)$, then if there is a way to use $v$ to extend a $K_p$ listed by $H(C)$ to a $K_{p+1}$, we will certainly find it. Similarly to the above analysis, using the routing algorithm of Theorem~\ref{thm-expander-routing} and the doubling procedure, we broadcast within $H(C)$ the edges incident to $v$ which are known to $H(C)$. This completes in $O(2^i / \mu_C+1)$ rounds, as the degree of $v$ is at most $2^i$.

We desire to bound the size of each $N^{+}_i(C)$ in order to conclude the proof. Let us compute an upper bound on the number of \emph{all} edges incident to nodes in $N^{+}(C)$. We wish to show that $\sum_{v \in N^{+}(C)} \deg(v) = \tilde O(n \cdot \mu_C)$. To do so, we split the edges into three categories: $E_1$ -- edges with both endpoints in $C$; $E_2$ -- edges with one endpoint in $C$; $E_3$ -- edges with both endpoints not in $C$. As $\mu_C$ is the average $C$-degree of the nodes in $C$, and $n$ is the number of nodes in the entire graph, implying $|C| \leq n$, it holds that $E_1 = O(n \cdot \mu_C)$. It is ensured in Lemma~\ref{lemma:decomp} that for every $v \in C$, it holds that $\deg(v) = \tilde O(\deg_C(v))$, where $\deg_C(v)$ is the $C$-degree of $v$, implying $|E_2| = \tilde O(|E_1|) = \tilde O(n \cdot \mu_C)$. Further, it is ensured in Lemma~\ref{lemma:decomp} that $|E_3|/n = \tilde O(|E_1|/|C|) = \tilde O(\mu_C)$, implying that $|E_3| = \tilde O(n \cdot \mu_C)$.
%It is ensured that the average $C$-degree in $N(C)$ is $\tilde{O}(\mu_C)$, by Lemma~\ref{lemma:decomp}. Thus, the average $C$-degree in $N^{+}(C)$ must also be $\tilde{O}(\mu_C)$.

Thus, for every $N^{+}_i(C)$, due to the pigeonhole principle, it must be that $|N^{+}_i(C)| = \tilde{O}(n \cdot \mu_C / 2^i)$. Further, as $n$ is the number of nodes in the graph, it also trivially holds that $|N^{+}_i(C)| \leq n$. All in all, we get that $|N^{+}_i(C)| = \tilde{O}(\min \{n, n \cdot \mu_C / 2^i\})$.

Finally, we can analyze the round complexity of the algorithm. The $K_p$ listing algorithm is shown in \cite{Censor+SODA21} to take $\tilde O(n^{1-2/p})$ rounds. For each $i$, the checking procedure in our Grover search takes $\tilde O(2^i / \mu_C+1)$ rounds. For every $i$ such that $2^i/\mu_C \leq 1$, the checking procedure takes $O(1)$, and $|N^{+}_i(C)| = \tilde O(n)$, implying that the Grover search takes a total of $\tilde O(n^{1/2})$ rounds, using Lemma~\ref{lemma:qsearchv0}. For every $i$ such that $2^i/\mu_C > 1$, the checking procedure takes $\tilde O(2^i / \mu_C+1) = \tilde O(2^i / \mu_C)$, and $|N^{+}_i(C)| = \tilde{O}(n \cdot \mu_C / 2^i)$, implying that the Grover search takes a total of $\tilde O(\sqrt{n \cdot \mu_C / 2^i} \cdot (2^i / \mu_C)) = \tilde{O}(\sqrt{n \cdot (2^i / \mu_C)})$ rounds, using Lemma~\ref{lemma:qsearchv0}. As $2^i = O(n)$ and $\mu_C = \Omega(n^{1/2})$ (due to the guarantees of the invocation of Lemma~\ref{lemma:decomp}, as stated above), this takes at most $\tilde O(n^{3/4})$ rounds.

We thus have that our quantum algorithm for detecting an instance of $K_{p+1}$ for $p\geq 5$ completes in $\tilde{O}(n^{3/4}+n^{1-2/p})$ rounds, with probability at least $1-1/\poly(n)$.

We note that we can decrease the $\tilde{O}(n^{3/4})$ part of the complexity, by slightly changing the listing algorithm of \cite{Censor+SODA21}. That is, the algorithm stated there performs $K_p$ listing in $\tilde O(n^{1-2/p})$ rounds, while ensuring $\mu_C = \Omega(n^{1/2})$. It is implied in the proofs in \cite{Censor+SODA21} that, for any $1/2 \leq \delta < 1$, one can pay an additional $\tilde O(n^\delta)$ rounds (by perform an exhaustive search, as done in Claim~\ref{claim:2hopNeighborhood}) in order to ensure $\mu_C = \Omega(n^{\delta})$. Further, notice that our Grover searches take a total of $\tilde O(n^{1/2} + n/\mu_C^{1/2}) = \tilde O(n^{1/2} + n^{1-\delta/2})$.

All in all, for any $1/2 \leq \delta < 1$, our algorithm requires $\tilde O(n^{1-2/p} + n^\delta + n^{1/2} + n^{1-\delta/2}) = \tilde O(n^{1-2/p} + n^\delta + n^{1-\delta/2})$ rounds. One can set $\delta = 2/3$, giving a final algorithm running in $\tilde O(n^{1-2/p} + n^{2/3} + n^{1-1/3}) = \tilde O(n^{1-2/p} + n^{2/3}) = \tilde O(n^{1-2/p})$ rounds, where the last transition is since $p \geq 6$.
\end{proof}


==> app_Congest_before_removing_k4.tex <==
\section{Missing Proofs from Section~\ref{sec:qcongest}}
\label{app:congest}

\subsection{Missing proof of Section \ref{subsec:triangles_congest}}
\label{appset_triangles_conget}
\begin{lemma-repeat}{lem:num_of_computation_units}
	In the process described in subsection~\ref{subsec:triangles_congest}, the set of marked computation units is pairwise-independent and is of size at least $\bar{n}/2$.
\end{lemma-repeat}
\begin{proof}
	We note that the set is indeed pairwise independent, as for each node $v$ the edges of the computation units with node $v$ are edge-disjoint.
	
	Recall that $m \leq c\bar{m}$ for some constant $c > 0$. Therefore, the number of edges in $|E\inext|$ is at least $\bar{m}/c$, and the average degree of $G\inext$ is at least $2\bar{m}/(cn\inext) \geq 2\bar{m}/\bar{n} = 2n^\delta$. Assume by contradiction that there are less than $\bar{n}/(2)$ computation units marked. Consider a graph $\tilde{G}$ that is defined by $G\inext$ after removing all edges participating in a marked computation unit. By the assumption there are at most $\bar{n}/(2) \lfloor \bar{n}^\delta/2c \rfloor$ edges removed, meaning that the number of edges in $\tilde{G}$ is at least $\bar{n}^{1+\delta}/(2c)$ edges remaining in $\tilde{G}$. This implies that the average degree in $\tilde{G}$ is at least $\bar{n}^\delta/2c$, meaning that there is at least one node $v$ with degree $\bar{n}^\delta/2c$, which contradicts the process above, as $v$ could have marked an additional computation unit.
\end{proof}

\paragraph{Correctness.}
If the graph is triangle-free then the network accepts, as a computation unit $v$ only rejects if it detects a triangle in the edges $E_1(v) \cup E_2^j(v)$ for some $1 \leq j \leq \bar{n}^{2/5}$. Otherwise, let $\{v_1,v_2,v_3\}$ be vertices of a triangle in $G'$. Let $i,j \in [\bar{n}^{2/5}]$ such that $v_1 \in A_i, v_2 \in A_j$ and let $P_{i,j}$ be the set of computation units that the pair $A_i,A_j$ is mapped to. Let $k \in [\bar{n}^{1/5}]$ and $r \in [\bar{n}^{1/5}]$ such that $v_3 \in S^{(r)}_k$ and let $w \in P_{i,j}$ be the computation unit in $P_{i,j}$ which $S_k$ is mapped to. We note that the triangle is contained in $E_1(w) \cup E^r_2(w)$, and therefore the network rejects in the protocol $A_r$, therefore the global protocol rejects as well. 



\subsection{Missing proofs from Section \ref{subsec:congestExtend}}
\label{app:congest:extend}

\subsubsection{Proof of Theorem \ref{thm:congest:four}}
\label{app:congest:extend:four}

\begin{theorem-repeat}{thm:congest:four}
\ThmCongestFour
\end{theorem-repeat}

To prove the theorem, we first prove the following theorem per cluster.

	Let $G = (V, E)$ be a graph, where $n = |V|$, and let $C = (V_C, E_C)$ be a cluster in an \emph{expander decomposition with high degree clusters (Definition~\ref{def:expanderDecompHighDeg})} of $G$. Denote by $N(C) \subseteq V \setminus V_C$ the set of nodes in $V \setminus V_C$ which have neighbors in $C$, and by $N^{+}(C) = N(C) \cup C$. Let $\bar E \subseteq (V_C \times N(C)) \cap E$, $E_{N(C)} \subseteq (N(C) \times N(C)) \cap E$ be sets of edges. Denote $k = |V_C|$, $q = |E_C|$, $\tilde {n} = |N(C)|$, $\tilde{m} = |E_{N(C)}|$, $\bar m = |\bar E|$, $\mu = q/k$. For any node $v \in N^{+}(C)$, denote by $\deg_{C}(v)$, $\deg_{N(C)}(v)$ the number of neighbors of $v$ in $V_C$, $N(C)$, respectively.

\newcommand{\ThmCongestPfour}
{
Let $a$, $b$ be any positive integers such that $a^2b = k$.
There exists an algorithm in the \qcongest model which detects the existence of an instance of $K_4$ in the graph $G' = (N^{+}(C), E_C \cup \bar E \cup E_{N(C)})$, which contains at least two nodes in $V_C$. The round complexity of the algorithm is $\tilde O((n/b + k/a) / \mu^{1/2} + (n/b + k/a)^{1/2} + a + b + 1)$, w.h.p. The algorithm uses only the edges $E_C \cup \bar E$ for communication. \dtodo{Note that the whp and the tilde are all in terms of $n$}
}

\begin{theorem}
	\label{thrm:k4:helper}
\ThmCongestPfour
\end{theorem}

\begin{proof}
	Primarily, as $C$ is a cluster in an \emph{expander decomposition with high degree clusters} (Definition~\ref{def:expanderDecompHighDeg}) of $G$, all of the following hold, by definition. These properties are crucial and widely used throughout the following proof.
	\begin{enumerate}
		\item The mixing time of $C$ is $\poly \log(n)$.
		%\item For every $v \in N(C)$, $\deg_C(v) \geq 1$.
		\item For every $v \in V_C$, $\deg_{N(C)}(v) = \tilde O(\deg_{C}(v))$. Further implying $\bar m = \tilde O(q)$.
		\item $\tilde{m}/n \leq m/n = \tilde O(q/k) = \tilde O(\mu)$.
		% \item For some value $\delta$, it holds that $\mu = \Omega(\delta)$.
	\end{enumerate}
	
	{\bf Triangle Listing.}
	Create a \emph{randomized} partition of $V_C$ into $a$ parts $V_C^1, \dots, V_C^a$, each of size $\tilde O(k/a)$, w.h.p., and of $N(C)$ into $N^{1}(C), \dots, N^b(C)$, each of size $\tilde O(\tilde{n}/b)$, w.h.p. Specifically, to create the partitions, every node in $v \in N^{+}(C)$ uniformly at random joins one of the parts, denoted $p(v)$, and sends $p(v)$ to all its neighbors in $V_C$, within $1$ round while using only the edges $E_C \cup \bar E$ for communication. Therefore, notice that for every edge $e = \{u, w\} \in E_C \cup \bar E$, both $u$ and $w$ know $p(u)$ and $p(w)$, and therefore we assume that this information is attached to $e$ from here on.
% \dtodo{fixed -- @keren, this used to be wrong before but now is right}.
	
	
%	\dtodo{elaborated this paragraph}
Create $k$ \emph{computation units} using the nodes $V_C$. The computational units can be viewed as some \emph{virtual nodes} which can communicate with one another and are simulated by $V_C$. Precisely, every node $v \in V_C$ with $\deg_C(v) = \Omega(\mu)$ creates $\Theta(\deg_C(v)/\mu)$ computational units which it simulates. Each computation unit can send and receive $\mu$ messages to and from any other computational unit in the cluster within $O(1)$ rounds. Observe that, by choosing appropriate constants, it can be ensured that there are exactly $k$ computational units simulated in $V_C$, as $\sum_{v \in V_C} \Theta(\deg_C(v)/\mu) = \Theta(q / \mu) = \Theta(k)$. Due to Claim~\ref{claim:2approx}, within $\poly \log (n)$ rounds, every node in $V_C$ can compute a $2$-approximation to the degree of every other node in $V_C$, and thus all the nodes in $V_C$ can know how many computational units are simulated at each node and which node simulates which units.
	
%	\dtodo{editted a bit}
Every computational unit is assigned exactly one triad (out of a total of $k$ triads) composed of two sets in the partition of $V_C$ and one set in the partition of $N(C)$. Let $v \in V_C$ be a node with at least one computational unit, and observe a single computational unit which is assigned to $v$, denoted $c_v$.  Denote by $V_C^i$, $V_C^j$ and $N^\ell (C)$ the sets corresponding to $c_v$, for some indices $i,j$ and $\ell$. The assignment of the sets to the computational units is hardcoded and is thus globally known. From here on and until the end of the proof, we continue with these specific $v$, $c_v$, $V_C^i$, $V_C^j$ and $N^\ell (C)$.
	
	Further, as the partitions are independent, we get that w.h.p., $|E(V_C^i, V_C^j)| = \tilde O(|E_C|/a^2 + 1) = \tilde O(q/a^2 + 1) = \tilde O(\mu k / a^2 + 1) = \tilde O(\mu b + 1)$, and, $|E(V_C^j, N^\ell (C))| = \tilde O(|\bar E|/(a\cdot b) + 1) = \tilde O(\bar m / (a \cdot b) + 1) = \tilde O(q / (a \cdot b) + 1) = \tilde O(\mu k / (a \cdot b) + 1) = \tilde O(\mu a + 1)$ (likewise with $|E(N^\ell (C), V_C^i)|$).
%\ktodo{please explain how we get these}\dtodo{fixed a small mistake and elaborated}.
	
	%\dtodo{elaborated on all the paragraph -- it is possible to slightly shorten the text here using Claim~\ref{claim:batchMessaging}, however, this is already written and so we might not want to touch it} 
	Thus, the unit $c_v$ can learn the edges $E(V_C^i, V_C^j)$, $E(V_C^j, N^\ell (C))$ and $E(N^\ell (C), V_C^i)$, within $\tilde O(a + b + 1)$ rounds, w.h.p., using only the $\mu$ bandwidth allocated by $v$ to $c_v$. To see this, notice that every edge which $c_v$ needs to learn is known to some node in $V_C$. Observe that the assignment of the sets to $c_v$ is known, the assignment of $c_v$ to $v$ is known, and for every edge in $e = \{u, w\} \in E \cup \bar E$, both $u$ and $w$ know to which sets $u$ and $w$ belong to. Thus, if $u \in V_C$ is incident to an edge $e$ which $c_v$ needs to learn, then $u$ knows to send $e$ edge to $v$. We showed that $c_v$ needs to receive at most $\tilde O(\mu a + \mu b + 1)$ messages. We now show that every $v$ needs to send at most $\tilde O(\deg_C(v) \cdot (a + b))$ messages. To see this, denote by $V_C^{\alpha(v)}$ the part such that $v \in V_C^{\alpha(v)}$, and let $e = \{v, w\} \in E_C$ and $e = \{v, u\} \in \bar E$ be edges incident to $v$, with the corresponding nodes $w \in V_C^{\alpha(w)}$ and $u \in N^{\beta(u)}(C)$. Notice that there are exactly $b$ computation units which are assigned both $V_C^{\alpha(v)}$ and $V_C^{\alpha(w)}$, implying that $e$ needs to be sent by $v$ to at most $b$ nodes. Similarly, exactly $a$ computational units are assigned both $V_C^{\alpha(v)}$ and $N^{\beta(u)}(C)$. Thus, in total, $v$ needs to send at most $O(\deg_C (v) \cdot b + \deg_{N(C)}(v) \cdot a) = \tilde O(\deg_C(v) \cdot (a+b))$ messages. Having shown the above constraints on how many messages each node sends and receives, by Theorem~\ref{thm-expander-routing}, this routing can be accomplished in $\tilde O(a + b + 1)$ rounds, w.h.p., as claimed.
	
	Notice that the algorithm up to this stage lists all $K_3$ involving at least two nodes in $V_C$, within $\tilde O(a + b + 1)$ rounds.\vspace{2mm}
	
\noindent{\bf Quantum Searches.}
	Create a degree-based partition of $N^{+}(C)$. Every node $u \in N^{+}(C)$ computes $f(u) = \deg_C(u)/a$, $g(u) = \deg_{N(C)}(u)/b$ \dtodo{address what happens when this is smaller than $1$}. Notice that $f(u)$ is an upper bound on the expected number of neighbors $u$ has in $V_C^i$, likewise in $V_C^j$, and $g(u)$ is a similar upper bound w.r.t. $N^\ell (C)$.  Finally, $u$ computes the value $h(u) = f(u) + g(u)$. It always holds that $h(u) \leq k/a + \tilde{n}/b \leq k / a + n / b$, it is possible to partition $N^{+}(C)$ into  $A_1, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ whereby $u \in A_{\lfloor \log (h(u)) \rfloor}$.
	
	Observe that $h(N^{+}(C)) = \sum_{u \in N^{+}(C)} h(u) = \sum_{u \in N^{+}(C)} \deg_C(u)/a + \deg_{N(C)}(u)/b = O((m + \bar m) / a + (\tilde{m} + \bar m) / b) = \tilde O(q / a + (\mu n + q) / b) = \tilde O(\mu k / a + ( \mu n + \mu k ) / b) = \tilde O(\mu k / a + \mu n /b)$, where the last transition is due to the fact that $k \leq n$, and the rest of the transitions follow from the properties of $C$ stated at the start of this proof.
	
	We iterate over all the sets $A_1, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ sequentially. Due to the fact that we desire to utilize the available bandwidth as much as possible, we treat nodes with low $h(\cdot)$ by coalescing them together, while those with high $h(\cdot)$ are dealt with in a different manner. As such, we have two different algorithms, for \emph{low-cost} and \emph{high-cost} nodes.\vspace{2mm}
	
\noindent{\bf Low-Cost Nodes.}
Iterate over the sets $A_1, \dots A_{\lfloor \log \mu \rfloor}$ sequentially. From here on, fix $\tau \in [\lfloor \log \mu \rfloor]$, and observe $A_\tau$.
	
	Construct an arbitrary BFS tree over $V_C \cup A_\tau$, which completes in $\poly \log (n)$ rounds, as the mixing time of $C$, and hence the diameter of $V_C \cup A_\tau$, is at most $\poly \log (n)$. Use this tree to number the nodes in $A_\tau$ from $1$ to $|A_\tau|$, and so, from now on, w.l.o.g., assume that the identifiers of the nodes in $A_\tau$ are in $[|A_\tau|]$.
	
	By definition, every node $v \in A_\tau$ satisfies $2^{\tau-1} < h(v) \leq 2^\tau$. Further, recall that $h(A_\tau) \leq h(N^{+}(C)) = \tilde O(\mu k / a + \mu n/b)$. Therefore, it is possible to create a partition of $A_\tau$ into $A_\tau^1, \dots, A_\tau^{k / a + n/b}$, whereby for every $\gamma \in [k / a + n/b]$, it holds that $h(A_\tau^j) = O(\mu + 2^\tau) = O(\mu)$, where the last transition holds as $\tau \leq \log \mu$. %\ktodo{Square brackets and $\{..\}$ in the calculations, what do they mean? Can they be replaces with the standard?}\dtodo{They do not mean anything special -- can be replaced. Will go over and replace when we have some downtime}
	
	%\dtodo{elaborated} 
	Perform a Grover search over $\gamma \in [k / a + n/b]$ to check whether an instance of $K_4$ exists which has at least two nodes in $V_C$ and involves at least one node from $A_\tau^\gamma$. Recall node $v \in C$ denoted above, along with $c_v$, $V_C^i$, $V_C^j$ and $N^\ell (C)$ . In order for $c_v$ to check if any $K_3$ which it sees using the edges between $V_C^i$, $V_C^j$ and $N^\ell (C)$ can be extended to a $K_4$ using a node from $A_\tau^\gamma$, it suffices for $c_v$ to learn the edges between all the nodes in $A_\tau^\gamma$ and each of these three sets. Denote by $\rho(i, j, \ell, \gamma)$ the number of such edges. Notice that $h(A_\tau^\gamma) = \tilde O(\mu)$ upper bounds the expectation of $\rho(i, j, \ell, \gamma)$. Thus, w.h.p., $c_v$ needs to receive $\tilde O(\rho(i, j, \ell, \gamma) + 1) = \tilde O(\mu + 1) = \tilde O(\mu)$ messages. Therefore, in total, $\tilde O(k \cdot \mu ) = \tilde O(q)$ messages need to be delivered, as there are $k$ computational units.
	
	
	\dtodo{begin remove} On the contrary, we need to show that $v$ sends at most $\tilde O(\deg_C(v) + 1)$ messages. \dtodo{complete routing}
	
	Having shown the above constraints on how many messages each node sends and receives, using Theorem~\ref{thm-expander-routing} this routing can be accomplished in $\tilde O(1)$ rounds, w.h.p. \dtodo{end remove}
	
	As the Grover search is over $\gamma \in [k / a + n/b]$, and checking for each $\gamma$ requires $\tilde O(1)$ rounds, w.h.p., the search can be performed in $\tilde O((k / a + n/b)^{1/2})$ rounds, w.h.p., using Lemma~\ref{lemma:qsearchv0}.\footnote{Notice that Lemma~\ref{lemma:qsearchv0} requires a \emph{leader} for the Grover search, however, as the diameter of $C$ is $\poly \log (n)$, this leader can be any arbitrary node within $C$, implying a round complexity cost which is multiplicative in $\poly \log (n)$.}\vspace{2mm}
	
\noindent{\bf High-Cost Nodes.} Iterate over the sets $A_{\lfloor \log \mu \rfloor + 1}, \dots, A_{\lceil \log (k / a + n / b) \rceil}$ sequentially. Fix $\tau \in [\lceil \log (k / a + n / b) \rceil] \setminus [\lfloor \log \mu \rfloor]$, and observe $A_\tau$.
	
    The current goal is to check for the existence of an instance of $K_4$ which contains at least two nodes in $V_C$ and one node in $A_\tau$.  Perform a Grover search over $w \in A_\tau$.
	% Recall node $v \in C$ denoted above, with its specific computational unit and the corresponding sets $V_C^i$, $V_C^j$ and $V_{\partial C}^\ell$ . In order for $v$ to check if any $K_3$ which it sees using the edges between $V_C^i$, $V_C^j$ and $V_{\partial C}^\ell$ can be extended to a $K_4$ using $w$, it suffices for $v$ to learn the edges between $w$ and each of these three sets.
	
	%\dtodo{elaborated} 
	Similarly to the \emph{Low-Cost} case, $c_v$ needs to learn the edges between $w$ and all the nodes in $V_C^i$, $V_C^j$ and $N^\ell (C)$. Denote by $\rho'(i, j, \ell, w)$ the number of such edges. Notice that $h(w) = O(2^\tau)$ upper bounds the expectation of $\rho'(i, j, \ell, w)$. Thus, w.h.p., $c_v$ needs to receive $\tilde O(2^\tau + 1)$ messages. Therefore, in total, $\tilde O(k \cdot (2^\tau + 1) )$ messages need to be delivered, as there are $k$ computational units.

	%\dtodo{added this} 
	On the contrary, for every edge $e = \{w, u\}$ incident to $w$, node $u$ sends $e$ to some node in $C$ which neighbors $u$. Observe now that all the edges incident to $w$ are known to the nodes of $C$. Given $e$, it is possible to compute all of the computational units which require $e$ if one knows the part in the partition to which $u$ belongs. This information is available, as $u$ can just attach the number of its part to $e$. Further, every node $x \in V_C$ receives at most $\deg(x) = \deg_C(x) + \deg_{N_C}(x) = \tilde O(\deg_C(x))$ such edges to be responsible for. As such, recalling that in total $\tilde O(k \cdot (2^\tau + 1) )$ messages need to be delivered, one can use the \emph{batch-messaging} algorithm from Claim~\ref{claim:batchMessaging} in order to deliver these messages within $\tilde O(k \cdot (2^\tau + 1) / q ) = \tilde O(2^\tau / \mu + 1) = \tilde O(2^\tau / \mu)$ rounds, w.h.p., where the last transition follows since $2^\tau = \Omega(\mu)$.
	
	 %\dtodo{explain the routing involved. First, node $w$ sends its edges into the cluster by having each of its nodes outside the cluster say that they neighbor $w$ to someone in the cluster -- this takes $O(1)$ rounds. Then, we can arbitrarily reshuffle the edges inside the cluster in order to be able to send them nicely. Perhaps have a general reshuffling theorem which can also be used above when we do the triangle listing stage}.
	
	 %Having shown the above constraints on how many messages each node sends and receives, using Theorem~\ref{thm-expander-routing} this routing can be accomplished in $O(2^\tau / \mu)$ rounds, w.h.p.
	
	As $h(N^{+}(C)) = \tilde O(\mu k / a + \mu n/b)$, we get that $|A_\tau| = \tilde O((\mu k / a + \mu n / b)/2^\tau)$. Thus, the Grover search takes $\tilde O(((\mu k / a + \mu n / b)/2^\tau)^{1/2} \cdot 2^\tau / \mu) = \tilde O((k / a + n / b)^{1/2} \cdot (2^\tau / \mu)^{1/2})$ rounds, w.h.p., using Lemma~\ref{lemma:qsearchv0}. As $2^\tau = O(n/b + k/a)$, we get a final complexity of $\tilde O((k / a + n / b)^{1/2} \cdot ((n/b + k/a) / \mu)^{1/2}) = \tilde  O((n/b + k/a) / \mu^{1/2})$.
\end{proof}


Using the above, we can now show the following main result. That is, given a specific cluster $C$, with corresponding $k$ and $\mu$, the following algorithm chooses the optimal $a$ and $b$ positive integers in order to execute the previous claim with.
\begin{theorem-repeat}{thm:congest:four}
\ThmCongestFour
\end{theorem-repeat}

\begin{proof}
	Primarily, we invoke the diameter reduction procedure described in Lemma~\ref{thm:diameter_reduce},which allows us to assume w.l.o.g. that $D$, the diameter of $G$, is at most $\poly \log (n)$.
	
	We proceed recursively,
	%apply the expander decomposition detailed in Lemma~\ref{lemma:decomp},
	and in each iteration we remove a constant factor of either the nodes or the edges, implying that we halt after at most $\poly \log (n)$ iterations.
	
	Perform the following algorithm for at most $\poly \log (n)$ iterations. First, compute the average degree of the graph, that is $\mu_G = \Theta(|E|/|V|)$, taking at most $O(D) = \poly \log (n)$ rounds.
	If $\mu_G \leq n^{4/9}$, then every node with degree at most $2n^{4/9}$ learns its induced 2-hop neighborhood, using Claim~\ref{claim:2hopNeighborhood}, in $O(n^{4/9})$ rounds, lists all the cliques it sees involving itself, and exits. In the case that this happens, it is ensured that at least half of the nodes in the graph exit at this iteration \dtodo{ref}.
	Otherwise, that is, if $\mu_G > n^{4/9}$, invoke the expander decomposition detailed in Lemma~\ref{lemma:decomp}. As $\mu_G > n^{4/9}$, by Lemma~\ref{lemma:decomp} it holds that for every   %and receive clusters which satisfy all of the properties required in Theorem~\ref{thrm:k4:helper} \dtodo{potentially extract to a definition}, with the additional constraint that for every
	cluster $C$ in the decomposition, the average degree in the cluster, $\mu_C$ satisfies $\mu_C = \Omega(n^{4/9})$.
	
	In the case that we run the expander decomposition, we proceed to detecting a $K_4$ which contains at least one edge inside one the clusters, if there exists such. Once we do this, it is possible to remove all the cluster edges from the graph, as removing them cannot remove an edge from any $K_4$ which was not already checked for. As the expander decomposition guarantees that at least a constant fraction of the edges are in the clusters, we can conclude the iteration.
	
	Therefore, we need to show how every cluster can detect a instance of $K_4$ which contains at least one edge inside the cluster, if there exists such. We run the following algorithm for each cluster. Observe that the algorithm only uses the edges inside the cluster as well as the edges crossing the cluster boundary (have exactly one endpoint in the cluster) for communication. This implies that all the clusters can execute the algorithm in parallel -- edges internal to a cluster are only used by it, and every edge between clusters is only used by two clusters, implying that we at most double the round complexity of the algorithm if all clusters run in parallel (i.e. we can assume w.l.o.g. that every cross-cluster edge sends on even round messages from the high end point to the low, and vice versa during odd rounds).
	
	%\dtodo{Try to play around with the numbers here, to see if we can get any better (see comment here): %https://www.wolframalpha.com/input/?i=minimize+max%281-b-x%2F2%2C+1-a-x%2F2%2C+a%2C+b%2C+x%29+where+2a%2Bb+%3D+1%2C+a+%3E%3D+0%2C+b+%3E%3D+0%2C+x+%3E%3D+0%2C+k%3D1%2C+w.r.t.+a%2C+b%2C+x
	%Note: It currently seems that $k=0.8$ is the big problem. If we assume $k\geq 0.9$, we get $21/45$ round complexity, and if we assume $k = 1$ we get $20/45$. For smaller $k$, we should let $a$ be bigger instead of setting $a = b$.
	%}
	
	Observe a specific cluster $C = (V_C, E_C)$ which we computed in the decomposition. Our goal is to detect any instance of $K_4$ in $G$ which contains at least two nodes in $V_C$. We break into cases depending on $k = |V_C|$.
	
	If $k = \tilde O(n^{2/5})$, then every node $v \in V_C$ learns its induced 2-hop neighborhood in $\tilde O(n^{2/5})$ rounds, using Claim~\ref{claim:2hopNeighborhood}.
	
	If $k = \omega(n^{2/5})$ and $k = \tilde O(n^{4/5})$, then set $b = n^{2/5}$, $a = k^{1/2}/n^{1/5}$. Observe that $a^2 b = k$, and that $a = k^{1/2}/n^{1/5} =  \omega(n^{1/5}/n^{1/5}) = \omega(1)$, implying that we can assume $a$ is an integer, as rounding it would not change its value by more than a constant factor. Therefore, we can execute Theorem~\ref{thrm:k4:helper} within $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b)$ rounds, w.h.p., where $\mu_C = \Theta(|E_C|/|V_C|)$. As stated above, due to the parameters we used, it is ensured that $\mu_C = \Omega(n^{4/9})$, and thus the total round complexity is $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b) = \tilde O((n^{3/5} + k^{1/2}n^{1/5})/n^{2/9} + (n^{3/5} + k^{1/2}n^{1/5})^{1/2} + k^{1/2}/n^{1/5} + n^{2/5}) = \tilde{O} (n^{3/5}/n^{2/9} + n^{3/10} + n^{1/5} + n^{2/5}) = \tilde O(n^{17/45})$, w.h.p., which is bounded by $\tilde O(n^{4/9})$.
	
	Finally, $k = \omega(n^{4/5})$ and $k \leq n = \tilde O(n)$. We set $b = n^{1/3}$, and $a = k^{1/2}/n^{1/6}$. Notice that $a^2 \cdot b = k$, and that $a = k^{1/2}/n^{1/6} =  \omega(n^{2/5}/n^{1/6}) = \omega(n^{7/30}) = \omega(1)$, implying that we can assume $a$ is an integer. Recall that $\mu_C = \tilde \Omega(n^{4/9})$. The total round complexity is thus $\tilde O((n/b + k/a) / \mu_C^{1/2} + (n/b + k/a)^{1/2} + a + b) = \tilde O((n^{2/3} + k^{1/2}\cdot n^{1/6}) / n^{2/9} + (n^{2/3} + k^{1/2}\cdot n^{1/6})^{1/2} + n^{1/3} + k^{1/2}/n^{1/6}) = \tilde O(n^{4/9} + n^{1/3} + n^{1/3}) = \tilde O(n^{4/9})$, w.h.p.
\end{proof}

\begin{comment}
\dtodo{DEPRECATED FROM HERE ON}
\dtodo{Sketch}

Given values $\delta$, $\kappa$, define the following algorithm. After we compute the expander decomposition (Step 2d in the algorithm), the algorithm works on a cluster-basis manner, and we denote the given cluster by $C$. Denote by $\partial C$ the nodes incident to $C$ -- that is, nodes which themselves are not in $C$, yet have neighbors in $C$. The algorithm only uses for communication the edges in $E(C, C)$ and $E(C, \partial C)$. For any node $v \in C \cup \partial C$, denote by $deg_C(v)$, $deg_{\partial C}(v)$ and $deg (v)$ the number of neighbors $v$ has in $C$, in $\partial C$, and in total, respectively. Note that it does not have to hold that the sum of the first two equals the third, as $C \cup \partial C$ does not necessarily cover all the nodes in the graph, however, for simplicity, we treat it as if the inequality does indeed hold.

\dtodo{Note: Unlike what we currently do with the algorithm in the SODA paper, here, we actually change the listing algorithm (for $K_3$) and make it run a bit slower. This overall makes us faster in terms of detection (for $K_4$) -- it is necessary in order to break below $o(n^{1/2})$.}

\begin{enumerate}
	\item For simplicity, execute the diameter reduction algorithm that Orr and Rotem mentioned to w.l.o.g. assume $D = \poly \log (n)$.
	\item While the graph is not empty:
	\begin{enumerate}
		\item Compute $\mu$, the average degree of the graph, in $O(D) = \poly \log (n)$ rounds.
		\item If $\mu \leq \delta$, then:
		\begin{enumerate}
			\item Any node $v$ where $deg (v) \leq 2 \delta$ learns its 2-hop neighborhood in $O(\delta)$ rounds, lists all the cliques which include itself, and removes itself and its incident edges from the graph.
			\item Go back to the beginning of the while loop. Analysis: in the step above, at least half of the nodes were removed from the graph, implying that we will reach this stage (and jump back to the start of the while loop) at most $\log n$ times.
		\end{enumerate}
		\item From here on, we can assume $\mu > \delta$.
		\item Compute an expander decomposition in $\poly \log n$ rounds. We now proceed to describe the algorithm for each cluster $C$.
		\item Denote $k = |C|$. If $k \leq \kappa$, every node in $C$ learns its 2-hop neighborhood in $\tilde O(\kappa)$ rounds (as the CS decomposition guarantees that for $v \in C$, it holds that $deg_{\partial C}(v) = \tilde O(deg_C(v))$), lists all the cliques involving itself, and the cluster is removed from the graph.
		\item Denote by $\mu_C$ and $\mu_{\partial C}$ the average degree of the nodes in $C$ and $\partial C$, respectively. If $\mu_C = o(\mu_{\partial C})$, or, if $\mu_C = o(\delta)$, then $C$ does nothing during the current iteration of the while loop. Using the proof of Claim 4.4 in SODA, plus the fact that $\mu > \delta$, it is possible to show that this step causes at most a constant fraction of the edges of the graph to be delayed to the next iteration. \dtodo{Note: In CPZ, they also remove nodes $v \in C$ from $C$ which are such that $deg_C(v) < deg_{\partial C}(v)$ -- this isn't necessary anymore since the CS decomposition guarantees that for $v \in C$, it holds that $deg_{\partial C}(v) = \tilde O(deg_C(v))$, which is good enough.}
		\item Let $a$, $b$ be two values which we define later. Split $C$ into $C_1, \dots, C_a$ uniformly at random, where $|C_i| = \tilde O(k /a)$ w.h.p.. Split $\partial C$ into $\partial C_1, \dots, \partial C_b$, where $|\partial C_i| = \tilde O(|\partial C|/b) = \tilde O(n/b)$. \dtodo{Notice that in the CPZ alg, $a = b = k^{1/3}$. We have to choose the values differently so that our detection algorithm will be faster.}
		\item We define $a^2b$ triads -- $C_i$, $C_j$, $\partial C_\ell$, where $i, j \in [a]$, $\ell \in [b]$. We later ensure that $a^2b = k$. Let $v \in C$. We assign to $v$ a number of triads which is $\Theta(deg_C(v)/\mu_C)$. Basically, this means that for every $\mu_C$ bandwidth (up to a constant) which $v$ has, it is assigned one triad. \dtodo{Orr gave this the notation of ``computational units''.} Therefore, from now on we will analyze how a single triad is dealt with using $\mu_C$ bandwidth, in order to let us ignore what happens at every specific node. Notice that every triad is assigned to one node in $C$, and that the assignment of triads to nodes in $C$ can be computed locally by every node in $C$ using tricks shown in CPZ.
		\item Let node $v$ be responsible for triad $C_i$, $C_j$, $\partial C_\ell$. It is possible that $v$ is responsible also for other triads, however, we assume that $v$ only allocates $\mu_C$ of its bandwidth in every round to dealing with this specific triad. Node $v$ learns the edges between the sets. This takes $O(\mu_C k / (\mu_C a^2)) = O(b)$ rounds to learn the edges between $C_i$ and $C_j$, and $\tilde O(\mu_C k / (\mu_C ab)) = \tilde O(a)$ rounds (since the number of edges crossing the boundary of $C$ is roughly at most the number of edges inside $C$, due to the cluster decomposition) to learn the edges between $\partial C_\ell$ and each of $C_i$, $C_j$. All in all, this step takes $O(a + b)$ rounds.
		\item Cluster $C$ splits the nodes in $\partial C$ into sets $\partial C^1, \dots \partial C^{\log n}$ \dtodo{In the part where we analyze the SODA algorithm, we use $\partial C_i$ for this notation, so change this part to match}, where $v \in \partial C^{i}$ if its degree is between $2^{i-1}$ and $2^i$. For each $i \in [\log n]$, do the following.
		\begin{enumerate}
			\item Grover search over node $w \in \partial C^i$. This takes $|\partial C^i|^{1/2}$ iterations of the following algorithm. Notice that $|\partial C^i| \cdot 2^i = O(\mu_C \cdot n)$, implying $|\partial C^i| = O(\mu_C \cdot n / 2^i)$.
			\begin{enumerate}
				\item We wish to see if it is possible to extend a $K_3$ which has been listed by $C$ to a $K_4$ using $w$.  \dtodo{We assume here that $w \in \partial C$, we also need to check for $w \in C$, but that should not be a problem}. To do so, we need to send the edges incident to $w$ to the nodes in $C$ which need them. To do so, we show one algorithm to send between $w$ and other nodes in $\partial C$, and one which deals with the edges between $w$ and nodes in $C$.
				\item First, the cluster broadcasts to $C \cup \partial C$ that we are searching over node $w$ now \dtodo{how does anyone know who $w$ is? Should be solvable, e.g. by $w$ choosing with some probability if it wants to go in this iteration, or something similar}. Then, every node which neighbors $w$ tells some node in $C$ about the edge between it and $w$. Thus, now all the edges in $E(\{w\}, C \cup \partial C)$ are known to nodes in $C$ \dtodo{need to reshuffle the edges so that each node in $C$ holds a number of edges proportional to its degree, etc -- arbitrary reshuffle is ok since the degree of a node from $C$ to other nodes in $C$ is at least roughly that as the number of neighbors it has in $\partial C$.}
				\item Let there be a specific triad $C_d$, $C_e$, $\partial C_f$, and $v$ the node responsible for the triad. W.h.p., $w$ neighbors $|\partial C_f| \cdot 2^i / |\partial C| = 2^i / b$ nodes in $\partial C_f$, requiring $\tilde O(2^i / (b \mu_C))$ rounds to deliver these edges to $v$ \dtodo{again, need some load balancing in terms of who sends which messages, but this is doable}. \dtodo{Total runtime that we get: $\tilde O(2^i / (b \mu_C))$ per iteration, and we have $O(\sqrt{\mu_C \cdot n / 2^i})$ iterations due to Grover. The product comes out to at most $O(n/(b \sqrt{\mu_C}))$ rounds.}
				\item \dtodo{Need to deal with the edges between $w$ and $C$ -- need to send them as well -- might require two different algorithms dependent on $k$....} \dtodo{We also have a small bug: for low $i$, we need to coalesce some nodes together when searching so that we don't waste bandwidth -- should not be a problem.}
			\end{enumerate}
		\item  \dtodo{In the end, we set $\kappa = \delta = b = n^{2/5}$, and this is also the round complexity which we get}
		\end{enumerate}

		
	\end{enumerate}
\end{enumerate}


\end{comment}


%%%
%%% p=7
%%%

\subsubsection{Proof of Theorem \ref{theorem:K6detectQcongest}}
\label{app:congest:extend:seven}

\begin{theorem-repeat}{theorem:K6detectQcongest}
\ThmCongestPseven
\end{theorem-repeat}

\begin{proof}
We begin by briefly explaining the $K_p$ listing algorithm of \cite{Censor+SODA21}. The algorithm of \cite{Censor+SODA21} works in iterations, which are composed of stages. In every stage, some $K_p$ in the graph may be listed.  We split the listed $K_p$ instances according to the stage in the algorithm in which they are listed. For each stage, we show how to detect in a quantum manner if there is an instance of $K_p$ that is listed in that stage which can be extended to (i.e., is a part of) an instance of $K_{p+1}$. As such, if there is any instance of $K_{p+1}$ in the graph, then we will certainly detect this as some instance of $K_p$ could be extended to it.

We now show the $K_p$ algorithm, and interject at appropriate places in order to perform quantum searches. Each iteration of the algorithm of \cite{Censor+SODA21} consists of the following steps.\vspace{2mm}
		
		\noindent{\bf Exhaustive search detection stage.} Every node $v$ with degree $O(n^{1/2})$ learns its induced 2-hop neighborhood in $O(n^{1/2})$ rounds using Claim~\ref{claim:2hopNeighborhood}, lists any cliques which it sees involving itself, and removes itself, along with its incident edges from the graph.
		
		\textbf{Detection of \boldmath{$K_{p+1}$}:} In particular, because the entire induced 2-hop neighborhood is learned, any instance of $K_{p}$ that is listed that can be extended to an instance of $K_{p+1}$ can be immediately listed in this way even without further communication, which proves our claim for this stage.\vspace{2mm}
		
		\noindent{\bf Graph decomposition and cluster exhaustive search detection stage.} An expander decomposition is computed according to Lemma~\ref{lemma:decomp}, while the above ensures that the average degree in the graph (and thus in the clusters, due to Lemma~\ref{lemma:decomp}) is at least $\Omega(n^{1/2})$. In clusters with $O(n^{1-2/p})$ nodes, each node learns its induced 2-hop neighborhood in $G$ using Claim~\ref{claim:2hopNeighborhood} and lists all the instances of $K_p$ which it is a part of, and finally removes itself and its incident edges from the graph. Because Lemma~\ref{lemma:decomp} promises that the number of edges that leave $C$ is at most $\tilde{O}(E_C)$, where $E_C$ are the edges inside $C$, and then this completes in $O(n^{1-2/p})$ rounds.
		
		\textbf{Detection of \boldmath{$K_{p+1}$}:}  As in the previous stage, because of the exhaustive search nature of this stage, we again obtain that any instance of $K_{p}$ that is listed that can be extended to an instance of $K_{p+1}$ can be immediately listed in this way even without further communication, which proves our claim for this stage.\vspace{2mm}
		
					
		\noindent{\bf Cluster listing.} Within every remaining cluster $C$, some nodes are designated as \emph{good} and the rest as \emph{bad}. Let $v$ be a good node. The nodes of $C$ learn amongst themselves all the edges in the 2-hop neighborhood of $v$. That is, the nodes of $C$ request from the nodes neighboring the cluster to send in edges from outside $C$ to nodes inside $C$, such that all the 2-hop neighborhood of $v$ is known to the nodes in $C$. Now, the nodes in $C$ ensure that every instance of $K_p$ involving $v$ and at least one other node in $C$ is becomes known to some node in $C$ -- that is, these $K_p$ instances are listed by $C$. The good nodes are then removed from the graph along with all of their edges. \vspace{3mm}

\noindent This concludes the description of the \congest algorithm in~\cite{Censor+SODA21}. The exact definition of good nodes is not required for our purpose.
%Also, we mention that during this stage, clusters whose average inner-degree is too small compared to average outer-degree of nodes neighboring the cluster are ignored and their edges are deferred to future iterations.
The proof of \cite{Censor+SODA21} shows that each iteration completes within $\tilde{O}(n^{1-2/p})$ rounds, and that after $\poly \log (n)$ iterations the remaining graph is empty and hence $\tilde{O}(n^{1-2/p})$ rounds are sufficient for the entire algorithm.\vspace{3mm}

		\noindent{\bf The cluster quantum detection stage.}
		We now provide the quantum procedure that we run after the above \textbf{Cluster listing} stage, in order to detect an instance of $K_{p+1}$ that contains an instance of $K_p$ that was listed during this stage. First, let the $C$-degree of a node be its number of neighbors in $C$,
%		recall that $n^{\delta} = n^{1/2}$ is a lower bound on
let $\mu_{C}$ be
		the average $C$-degree of nodes in $C$, and let $H(C)$ be the high $C$-degree cluster nodes, namely, those of $C$-degree $
		%\Omega(n^{\delta}) = \Omega(n^{1/2})$.
\Omega(\mu_{C})$.  Notice that due to the invocation above of Lemma~\ref{lemma:decomp}, it holds that $\mu_C = \Omega(n^{1/2})$.
		A more precise description of the algorithm in~\cite{Censor+SODA21} is that the 2-hop neighborhood of each good node $v$ becomes known to the nodes in $H(C)$ rather than to any node in $C$. Second, denote by $N^{+}(C)$ the set of nodes which have a neighbor in $C$ (this includes all of $C$ as $C$ is connected, by definition) and by $N(C) = N^{+}(C)-C$ the neighbors of $C$ outside of $C$. In the above \textbf{Cluster listing} stage we piggyback the degree (not $C$-degree) of every node in $N(C)$ onto the messages containing its edges, so that the degrees of all nodes in $N(C)$ are also known to nodes of $H(C)$.
		
The quantum process starts with the following. The nodes in $C$ elect some arbitrary leader $v_C \in H(C)$.
%and construct a virtual binary tree $T_C$ rooted at $v_C$ which spans $H(C)$, and has depth at most $\poly \log (n)$.
This can be done in $\poly \log (n)$ rounds because this is a bound on the diameter of the cluster, by Lemma~\ref{lemma:decomp}. The nodes of $H(C)$ now broadcast within $H(C)$ the degrees of all the nodes in $N(C)$. This is done in two steps. In the first step, each node in $H(C)$ sends $v_C$ the degrees of nodes in $N(C)$ which it knows about.
%Then, every node tells $v_C$ about the degrees of nodes in $N(C)$ which it knows about.
As every node sends and receives at most $|N(C)| = O(n)$ pieces of information, and every node in $H(C)$ has $C$-degree at least $\Omega(\mu_C) = \Omega(n^{1/2})$, this takes at most $\tilde O(n^{1/2})$ rounds, using the routing algorithm of Theorem \ref{thm-expander-routing}. In the second step, $v_C$ makes this information known to all nodes in $H(C)$ using a simple doubling procedure: in each phase of this procedure, each informed node shares the information with a unique uninformed node. Each phase completes in $\tilde O(n^{1/2})$ rounds by the same argument using the routing algorithm of Theorem~\ref{thm-expander-routing}, and the number of phases is logarithmic. In a similar fashion, the nodes in $H(C)$ learn all the degrees of the nodes in $C$.
%Finally, the information is broadcast to all of $H(C)$ over $T_C$ \ktodo{Do we actually need to reference the SPAA21 paper? This looks trivial to me.}. In a similar manner, the nodes of $H(C)$ also broadcast amongst themselves the $C$-degrees of all nodes in $C$. \dtodo{This seems like some stuff is repeated in the paragraph multiple times.}

Knowing the degrees of all nodes in $N^{+}(C)$, the nodes $H(C)$ \emph{bucket} $N^{+}(C)$ by degrees. That is, they compute $N^{+}(C) = N^{+}_1(C), \dots, N^{+}_{\log n}(C)$, such that the degree of any $v \in N^{+}_i(C)$ is in $[2^{i-1},\dots,2^i)$. We iterate over the $\log n$ buckets, whereby in each bucket we check whether a node in $N^{+}_i(C)$ can be used to extend some $K_p$ instance, which is already listed by $H(C)$, into an instance of $K_{p+1}$. This is done as follows.

Fix an $i$ between 1 and $\log n$. We perform a Grover search over $v \in N^{+}_i(C)$ using $v_C$ as the leader of the search: In each query (i.e., over such a $v$), we broadcast within $H(C)$ all the neighbors of $v$ which are known to $H(C)$, in order to try to extend any $K_p$ listed by $H(C)$ to a $K_{p+1}$ involving $v$. Let $\kappa_{p}$ be such a $K_p$. As it is listed by $H(C)$, it must involve at least one good node in $C$, denoted $g \in \kappa_{p}$. Further, recall that every edge in the 2-hop neighborhood of $g$ is known to $H(C)$. Thus, if $v$ that can be used to extend $\kappa_{p}$ to an instance of $K_{p+1}$, all the edges between $v$ and $\kappa_{p}$ are known to the nodes of $H(C)$. Therefore, if we manage to broadcast in $H(C)$ all the edges incident to $v$ that are known to $H(C)$, then if there is a way to use $v$ to extend a $K_p$ listed by $H(C)$ to a $K_{p+1}$, we will certainly find it. Similarly to the above analysis, using the routing algorithm of Theorem~\ref{thm-expander-routing} and the doubling procedure, we broadcast within $H(C)$ the edges incident to $v$ which are known to $H(C)$. This completes in $O(2^i / \mu_C+1)$ rounds, as the degree of $v$ is at most $2^i$.

We desire to bound the size of each $N^{+}_i(C)$ in order to conclude the proof. Let us compute an upper bound on the number of \emph{all} edges incident to nodes in $N^{+}(C)$. We wish to show that $\sum_{v \in N^{+}(C)} \deg(v) = \tilde O(n \cdot \mu_C)$. To do so, we split the edges into three categories: $E_1$ -- edges with both endpoints in $C$; $E_2$ -- edges with one endpoint in $C$; $E_3$ -- edges with both endpoints not in $C$. As $\mu_C$ is the average $C$-degree of the nodes in $C$, and $n$ is the number of nodes in the entire graph, implying $|C| \leq n$, it holds that $E_1 = O(n \cdot \mu_C)$. It is ensured in Lemma~\ref{lemma:decomp} that for every $v \in C$, it holds that $\deg(v) = \tilde O(\deg_C(v))$, where $\deg_C(v)$ is the $C$-degree of $v$, implying $|E_2| = \tilde O(|E_1|) = \tilde O(n \cdot \mu_C)$. Further, it is ensured in Lemma~\ref{lemma:decomp} that $|E_3|/n = \tilde O(|E_1|/|C|) = \tilde O(\mu_C)$, implying that $|E_3| = \tilde O(n \cdot \mu_C)$.
%It is ensured that the average $C$-degree in $N(C)$ is $\tilde{O}(\mu_C)$, by Lemma~\ref{lemma:decomp}. Thus, the average $C$-degree in $N^{+}(C)$ must also be $\tilde{O}(\mu_C)$.

Thus, for every $N^{+}_i(C)$, due to the pigeonhole principle, it must be that $|N^{+}_i(C)| = \tilde{O}(n \cdot \mu_C / 2^i)$. Further, as $n$ is the number of nodes in the graph, it also trivially holds that $|N^{+}_i(C)| \leq n$. All in all, we get that $|N^{+}_i(C)| = \tilde{O}(\min \{n, n \cdot \mu_C / 2^i\})$.

Finally, we can analyze the round complexity of the algorithm. The $K_p$ listing algorithm is shown in \cite{Censor+SODA21} to take $\tilde O(n^{1-2/p})$ rounds. For each $i$, the checking procedure in our Grover search takes $\tilde O(2^i / \mu_C+1)$ rounds. For every $i$ such that $2^i/\mu_C \leq 1$, the checking procedure takes $O(1)$, and $|N^{+}_i(C)| = \tilde O(n)$, implying that the Grover search takes a total of $\tilde O(n^{1/2})$ rounds, using Lemma~\ref{lemma:qsearchv0}. For every $i$ such that $2^i/\mu_C > 1$, the checking procedure takes $\tilde O(2^i / \mu_C+1) = \tilde O(2^i / \mu_C)$, and $|N^{+}_i(C)| = \tilde{O}(n \cdot \mu_C / 2^i)$, implying that the Grover search takes a total of $\tilde O(\sqrt{n \cdot \mu_C / 2^i} \cdot (2^i / \mu_C)) = \tilde{O}(\sqrt{n \cdot (2^i / \mu_C)})$ rounds, using Lemma~\ref{lemma:qsearchv0}. As $2^i = O(n)$ and $\mu_C = \Omega(n^{1/2})$ (due to the guarantees of the invocation of Lemma~\ref{lemma:decomp}, as stated above), this takes at most $\tilde O(n^{3/4})$ rounds.

We thus have that our quantum algorithm for detecting an instance of $K_{p+1}$ for $p\geq 5$ completes in $\tilde{O}(n^{3/4}+n^{1-2/p})$ rounds, with probability at least $1-1/\poly(n)$.

We note that we can decrease the $\tilde{O}(n^{3/4})$ part of the complexity, by slightly changing the listing algorithm of \cite{Censor+SODA21}. That is, the algorithm stated there performs $K_p$ listing in $\tilde O(n^{1-2/p})$ rounds, while ensuring $\mu_C = \Omega(n^{1/2})$. It is implied in the proofs in \cite{Censor+SODA21} that, for any $1/2 \leq \delta < 1$, one can pay an additional $\tilde O(n^\delta)$ rounds (by perform an exhaustive search, as done in Claim~\ref{claim:2hopNeighborhood}) in order to ensure $\mu_C = \Omega(n^{\delta})$. Further, notice that our Grover searches take a total of $\tilde O(n^{1/2} + n/\mu_C^{1/2}) = \tilde O(n^{1/2} + n^{1-\delta/2})$.

All in all, for any $1/2 \leq \delta < 1$, our algorithm requires $\tilde O(n^{1-2/p} + n^\delta + n^{1/2} + n^{1-\delta/2}) = \tilde O(n^{1-2/p} + n^\delta + n^{1-\delta/2})$ rounds. One can set $\delta = 2/3$, giving a final algorithm running in $\tilde O(n^{1-2/p} + n^{2/3} + n^{1-1/3}) = \tilde O(n^{1-2/p} + n^{2/3}) = \tilde O(n^{1-2/p})$ rounds, where the last transition is since $p \geq 6$.
\end{proof}


==> app_cycles.tex <==
\section{Missing Proofs from Section~\ref{sec:cycles}}
\label{app:cycles}

\subsection{Odd-length cycles}
\label{app:cycles:odd}

For odd-length cycles $C_{\ell}$, our algorithm is quite simple:
the optimal \emph{classical} algorithm goes over the network nodes one-by-one, and essentially uses an $O(\ell)$-round BFS (more precisely, a color-coded BFS, as detailed below)
to search 
for an $\ell$-cycle starting from each node.
Using Grover search, we can perform this process faster: instead of $n$ classical ``queries'' (one for each node),
we perform $\sqrt{n}$ quantum ``queries'', each requiring constant rounds to evaluate.

\begin{theorem-repeat}{thm:Codd-lb}
	\OddCycleLB
\end{theorem-repeat}

\begin{proof}
Drucker et al. \cite{DKO14} showed that for any odd constant $\ell\ge 5$, an $r$-round distributed algorithm for $C_\ell$-detection can be converted into a 2-party $r$-round $\tilde O(rn)$-bit protocol for computing the disjointness function on $\Theta(n^2)$-bit strings. This reduction is actually a black-box reduction, which also holds in the quantum setting: an $r$-round distributed quantum algorithm for $C_\ell$-detection can be converted into a 2-party $r$-round $\tilde O(rn)$-qubit quantum protocol for computing the disjointness function on $\Theta(n^2)$-bit strings.

It is known that any $r$-round 2-party quantum protocol for he disjointness function on $\Theta(n^2)$-bit strings requires $\tilde \Omega(n^2/r+r)$ qubits of communication \cite{BGK+18}. We thus obtain the lower bound $rn=\tilde \Omega(n^2/r+r)$, which implies the lower bound $r=\tilde\Omega(\sqrt{n})$ on the round complexity of any quantum algorithm for $C_\ell$ detection in the \qcongest model.
\end{proof}


\subsection{Even-length cycles}
\label{app:cycles:even}
For even cycles, we can go below $O(\sqrt{n})$ rounds, just as in the classical model we can go below $O(n)$.
The formal statement of our result for even cycles is the following:
%\ftodo{The counter of the following theorem is set manually to display ``Theorem 4''. Check that the number is correct before submitting.}
%\begin{theorem-repeat}{th:cycle-even}
\addtocounter{theorem}{-25}
\begin{theorem}[repeated]
	For any constant 
	$k \geq 2$,
	there is a $\QCONGEST$ algorithm that runs in $\tilde{O}(n^{1/2 - 1/(2k(k-1))})$
	rounds, and solves the $C_{2k}$-freeness problem with probability $1 - 1/\mathrm{poly}(n)$.
\end{theorem}
\addtocounter{theorem}{+25}
%	\label{thm:C2k}
%\end{theorem-repeat}

%\ktodo{Move from here and below to Appendix \ref{app:cycles:even} (file app\_cycles.tex) and replace with a sketch.}

Next we introduce the ingredients that go into the algorithms, and analyze their correctness and their running time.

\paragraph{Color-coded BFS.}
Our algorithm uses color-coded BFS \cite{AYZ97} to search for $2k$-cycles.
The color-coded BFS is given the following information:
\begin{itemize}
	\item A set $A \subseteq V$ of \emph{active nodes}, which are the nodes that will participate in the BFS.
		Each node knows whether it is active or not.
	\item A set of \emph{sources}, $S \subseteq A$, such that each node knows whether it is in $S$ or not.
	%\item Each source node $v \in S$ has an initial color, $c(v) \in \set{ 0,\bot}$,
		%with ``0'' meaning that we want to assign sources the color 0, and ``$\bot$'' meaning
		%we want to assign them a random color.
	\item For each node $v \in A$, a \emph{height} $h(v) \in \mathbb{N}$, known to node $v$ and its neighbors.
		This is optional; if no heights are given, we assume $h(v) = 0$ for all $v \in A$.
	\item A bound $M \in \mathbb{N}$ on the allowable congestion per node.
\end{itemize}

The color-BFS consists of $O(k^k)$ repetitions of the following steps:
\begin{itemize}
	\item We assign to each
		%non-source node $v \in A \setminus S$, and to each source node $v \in S$
		%with an initial color assignment of $c(v) = \bot$,
		active node $v \in A$
		a uniformly random color $c(v) \in \set{0,\ldots,2k-1}$.
	\item Each source node $v \in S$ whose color is $c(v) = 0$
		sends its ID to all neighbors with colors 1 or $2k-1$,
		whose height is no greater than $v$'s 
       %(i.e., to the set $\set{ w \in N(v) \stt h(w) \leq h(v) \wedge c(w) \in \set{1,2k-1} }$.
       (i.e., to the set $\{ w \in N(v) \stt h(w) \leq h(v) \textrm{ and } c(w) \in \set{1,2k-1} \}$.
	\item Next, we execute $k - 1$ phases, with each phase taking $M$ rounds.
		In phase $i \in \set{1,\ldots,k-1}$,
		active nodes with color $i$ or $2k - i$ forward the first $M$ IDs that they received
		to their neighbors with color $i + 1$ or $2k-i-1$, respectively.
	\item Finally, if some active node $v$ with color $k$ receives the same ID from two neighbors
		with colors $k - 1$ and $k+1$ respectively,
		then $v$ informs the leader that a $2k$-cycle has been found.
\end{itemize}
The leader returns ``yes'' iff it was informed of a $2k$-cycle by some node.

Define the \emph{congestion} $m(v)$ at a node $v \in A$
to be the maximum number of IDs that node $v$ may need to forward during a given iteration of the search,
regardless of $v$'s color.
That is,
$m(v)$ is the number of nodes $w \in S$
such that there is a path $w = w_0,\ldots,w_{\ell} = v$ of active nodes,
with $1 \leq \ell \leq k-1$,
from $w = w_0$ to $v = w_{\ell}$,
where $h(w) \geq h(w_1)$ (recall that source nodes only send their IDs to nodes of equal-or-lesser height).

The color-coded BFS requires $O(k M)$ rounds, and it has the following properties:
\begin{itemize}
	\item If the network does not contain a $2k$-cycle, then the leader returns ``no''.
	\item If the network contains a $2k$-cycle $u_0,\ldots,u_{2k-1}$ such that
		$h(u_0) \geq \max_{i = 1,\ldots,2k-1} h(u_i)$,
		and every cycle node $u_i$ has congestion $m(u_i) \leq M$,
		then with probability $99/100$ the leader returns ``yes''.
\end{itemize}

\subsubsection{Ruling Out Dense Graphs}
As in \cite{FGKO18,EFFKO19}, we rely on the well-known result from extremal combinatorics (see, e.g., \cite{BZ17}) that any graph that is $C_{2k}$-free
has at most $c_k n^{1-1/k}$ edges, where $c_k$ is a constant (which may depend on $k$, but not on $n$). 
At the beginning of the algorithm, the network leader counts the edges in the graph, and if there are more than $c_k n^{1-1/k}$ edges, we immediately reject.
In the sequel we assume that $|E| \leq c_k n^{1-1/k}$.

%sub-square root round complexity \TODO{can we say sub-square root?}. First, using the diameter decomposition of \TODO{cite}, we may assume w.l.o.g. that the diameter of the graph is $O(\log{n})$ \TODO{more details are needed here}. We call the node with the highest id in the network the network leader. Using standard arguments, in $O(D)$ rounds all nodes in the network learns the identifier of the node $v^*$. 

%\TODO{both light and heavy procedures uses an identical sub-procedure which given some subnetwork, a coloring and orientation on edges determine whether there is a $2k$-colored vertex that is in a sort-of-directed $2k$-cycle. Maybe merge?}

\subsubsection{Searching for Heavy Cycles}
Fix a threshold $n^{\delta}$, where $\delta \in (0,1)$, and let us say that node $v \in V$ is \emph{heavy} if $\deg(v) \geq n^{\delta}$.
Since we assume that $|E| \leq c_k n^{1-1/k}$, the network contains at most $O(n^{1-1/k-\delta})$ heavy nodes.
Let $V_H \subset V$ be the set of heavy nodes, and let $V_L = V \setminus V_H$ be the set of light (i.e., non-heavy) nodes.

A cycle $v_1,\ldots,v_2k$ is called a \emph{heavy cycle} if it contains at least one heavy node.
We search for heavy $C_{2k}$-cycles as follows:
\begin{enumerate}
	\item We collect the IDs of the heavy nodes in $V_H$ up the spanning tree, and the leader then broadcasts $V_H$ to the entire network.
		Each heavy node $v \in V_H$ orders the IDs in $V_H$ in some pre-determined manner,
		$V_H = \set{v_1,\ldots,v_{\ell}}$,
		and
		computes its rank $r(v) \in [|V_H|]$ in the ordering.
		(That is, if $v = v_i$, then $r(v) = i$.)
	\item We perform a Grover search,
		to search for a heavy node that participates in a $C_{2k}$. 

		The query performed inside the Grover search is a color-coded BFS
		using a single heavy node as the source.
		Specifically, for each $i = 1,\ldots,|V_H|$,
		let $A_i$ be the execution of color-coded BFS
		using $S = \set{v_i}$, with all nodes active, congestion bound $M = 1$, and no heights used.
		%Let us define the query performed inside the Grover search.
		%Define a sequence of algorithms $A_1,\ldots,A_{\ell}$ (where $\ell = |V_H|$) as follows:
		%algorithm $A_i$ executes in $k - 1$ rounds.
		%In the first round, node $v_i$ sends a token to all its neighbors, while all other nodes remain silent.
		%In each subsequent round $j = 1,\ldots,k-1$, all nodes with color $j$ or $2k - j$ 
		%that received the token in the previous round (i.e., round $j - 1$)
		%forward the token to all their neighbors.
		%Finally, if in the last round some node colored $k$ receives the token from two neighbors with colors $k-1$
		%and $k+1$, respectively, then $A_i$ rejects.
		%\TODO{Presumably the leader need to be informed?}

		The graph performs a Grover search over $i = 1,\ldots,|V_H|$,
		to find some $i$ such that $A_i$ outputs ``yes'', or determine that there is no such $i$.
		If we find an $i$ such that $A_i$ outputs ``yes'', 
		then the leader announces the graph is not $C_{2k}$-free
		and we halt.
		\item If we have not halted so far, we announce that the graph is $C_{2k}$-free.
		\end{enumerate}

Following this part of the algorithm, all heavy nodes ``deactivate'', in the sense that
we no longer search for cycles containing them.
However, they still participate in managing the Grover search.

\paragraph{Correctness.}
Suppose that there is a heavy $2k$-cycle $u_0,\ldots,u_{2k-1}$ in the graph, and assume w.l.o.g.\ that $u_0$
 is a heavy node.
 Let $i$ be such that $u_0 = v_i$.
 Since we perform each color-coded BFS with only one source,
 the congestion bound of 1 suffices for all nodes to forward the source's ID.
 Thus, with probability $99/100$, we will find the cycle.

\paragraph{Runtime.}
The running time of this part of the algorithm is $O( \sqrt{n^{1-1/k-\delta}} )$,
since we are searching over the heavy nodes, of which there are $n^{1-1/k-\delta}$,
and the query itself requires a constant number of rounds.
Plugging in $\delta = (k-2)/(k(k-1))$,
we get a running time of
$O(n^{1/2 - 1/(2k(k-1))})$.

\subsubsection{Searching for Light Cycles}
To search for a cycle that does not contain a heavy node, the network first attempts to compute an $O(n^{1/k})$-forest decomposition of the light nodes, using the procedure of \cite{BM08}. This is a partition of the vertices in $V_L$ into layers $V_L^1,\ldots,V_L^t$,
where $t = O(\log n)$, such that for each $i = 1,\ldots,t-1$, any node $v \in V_L^i$ has at most $O(n^{1/k})$ edges to nodes
in $\bigcup_{j \geq i} V_L^i$.
It is known that a $C_{2k}$-free graph admits an $O(n^{1/k})$-forest decomposition,
so if we fail to compute the forest decomposition, we reject (as in \cite{FGKO18,EFFKO19}).

Define the \emph{height} $h(v)$ of a node $v \in V_L$ to be the number $i$ of the layer $V_L^i$ such that $v \in V_L^i$.

\paragraph{Intuition.}
Classically, we now search for a $2k$-cycle as follows (as in \cite{FGKO18,EFFKO19}):
we assign each light node $v$ a random color $c(v) \in \set{0,\ldots,2k-1}$,
and search for cycles $u_0,\ldots,u_{2k-1}$ such that $c(u_i) = i$ for each $i$,
and additionally, $u_0$ is at least as high as all other cycle nodes.
To do so, we have all nodes $v$ with color 0 broadcast the ID to their neighbors $w \in N(v)$
whose height is no greater than $v$'s.
Note that each node $w$ receives at most $O(n^{1/k})$ IDs in this step,
because $w$ has at most that many neighbors with equal-or-greater height to $w$'s.
Next, we carry out a color-coded BFS, with the nodes of each color forwarding all IDs they received to the nodes of the next color.
The total number of IDs that may be sent at any point is bounded by $O(n^{1/k+(k-2)\delta})$:
in the first step, at most $O(n^{1/k})$ IDs are received, and in each of the subsequent $k - 1$ steps,
this is multiplied by at most the degree of a
light node, which is at most $n^{\delta}$.

To speed up this procedure using a Grover search, we have each node $v$ choose a random index $s(v) \in [n^{\alpha}]$,
where $\alpha > 1$ is a parameter.
We then search over the indices $i \in [n^{\alpha}]$, to find a cycle $u_0,\ldots,u_{2k-1}$ such that $s(u_0) = i$.
By partitioning the nodes among the indices in this way, we reduce the congestion:
in each color-BFS, we will have to forward at most $O(n^{1/k+(k-2)\delta - \alpha})$
IDs in expectation, because each of the possible sources chooses that particular index with probability $n^{-\alpha}$.
The Grover search will therefore cost
$O(\sqrt{n^{\alpha}} \cdot n^{1/k + (k-2)\delta - \alpha}) = O(n^{1/k + (k-2)\delta - \alpha/2})$
rounds in total, and we can choose $\alpha,\delta$ so that this comes out to $o(\sqrt{n})$.

The parameters are set as follows.
First, we choose $\alpha$ so that the expected congestion during the search comes out to a constant:
\begin{equation*}
	\alpha = 1/k + (k-2)\delta.
\end{equation*}
We point out that it is better to have a finer partition (larger $\alpha$), because 
the congestion is reduced by a factor of $n^{-\alpha}$, while we pay only $n^{\alpha/2}$ for the search over the indices.
Under this choice of $\alpha$,
the entire quantum search for light cycles costs $O(n^{\alpha/2}) = O(n^{(1/k + (k-2)\delta)/2})$.

Next, we set $\delta$ so as to balance the cost of searching for heavy and light cycles:
\begin{equation*}
	\frac{1-1/k-\delta}{2} = \frac{1/k + (k-2)\delta}{2}.
\end{equation*}
Solving for $\delta$ yields
\begin{equation*}
	\delta = \frac{k-2}{k(k-1)}.
\end{equation*}
The resulting running time is
$O(n^{1/2 - 1/(2k(k-1))})$.
%\begin{equation*}
	%\frac{1}{2}\left( \frac{k-1}{k} - \frac{k-2}{k(k-1)} \right)
	%=
	%\frac{1}{2}\left( \frac{k^2+2k-1 - k + 2}{k(k-1)} \right)
	%=
	%\frac{1}{2}\left( \frac{k^2 - k + 1}{k^2 - k} \right)
	%=
	%\frac{1}{2} \cdot \left( 1 - \frac{1}{k^2 - k} \right).
%\end{equation*}


\paragraph{Formal statement of the quantum search.}
Before we begin the search, each light node $v \in V_L$ assigns itself a random index $s(v) \in [n^{\alpha}]$,
where $\alpha = 1/k + (k-2)\alpha$.
We now search over the indices $[n^{\alpha}]$.
The classical query $A_i$ for a given index $i \in [n^{\alpha}]$ is a color-coded BFS, with the following parameters:
\begin{enumerate}
	\item The active nodes are all light nodes, $V_L$.
	\item The set $S$ of sources is the set of light nodes with index $i$,
		i.e., $\set{ v \in V_L \stt s(v) = i}$.
	\item The heights are as defined above --- $h(v)$ is the index of the layer in the forest decomposition that contains $v$.
	\item The congestion bound is $M = a \log n$, where $a > 1$ is a constant to be determined later.
\end{enumerate}

\paragraph{Correctness.}
Suppose there is a $2k$-cycle $u_0,\ldots,u_{2k-1}$ consisting only of light nodes,
and assume w.l.o.g.\ that $h(u_0) \geq \max_{i = 1,\ldots,2k-1} h(u_i)$.
Then $A_{s(u_0)}$ will find the cycle with constant probability, 
if the congestion at each cycle node is no greater than our congestion bound of $M = a \log n$.
We show that when $\alpha = 1/k + (k-2)\delta$, this holds with constant probability.

To bound the congestion at any active node $u$,
let us first count the \emph{good paths}, $\pi = w_0,\ldots,w_{\ell} = u$,
where $w_0,\ldots,w_{\ell} \in A$,
$1 \leq \ell \leq k-1$, $w_0 \in S$, and $h(w_0) \geq h(w_1)$.
For each $j \leq \ell - 1$, the
number of paths $w_j,\ldots,w_{\ell} = u$ of light nodes is at most $n^{\delta \cdot j}$.
As for the first step in the path, each node $w_1$ has at most $n^{1/k}$ neighbors $w_0$
with $h(w_0) \geq h(w_1)$, by the properties of the forest decomposition.
All together, we see that there are at most $n^{1/k + (k-2)\delta}$
good paths to $u$.
However, not all these paths start at a \emph{source node}:
the first node $w_0$ of the path chooses a random index $s(w_0) \in [n^{\alpha}]$,
and participates as a source only when we query that particular index.

Let $P(u) \subseteq A$ be the set of nodes that have a good path to $u$.
As we said above, $|P(u)| \leq n^{1-1/k +  (k-2)\delta}$. (We counted \emph{paths} rather than
 \emph{distinct nodes} above, and this may lead to over-counting, but since we need only an upper bound, this is not a problem.)
 Each node in $P(u)$ assigns itself a random index in $[n^{\alpha}]$,
 and since $\alpha = 1-1/k + (k-2)\delta$,
 in expectation, exactly one node chooses each index.
 By Chernoff, if we choose the constant $a$ high enough,
 then with probability $1 - 1/\mathrm{poly}(n)$,
 no index will be chosen by more than $a \log n$ nodes in $P(u)$,
 and the congestion bound will be obeyed.
 

\paragraph{Runtime.}
Computing the forest decomposition requires $O(\log n)$ rounds.
Afterwards, we execute an unnested quantum search over the search space $n^{\alpha} = n^{1-1/k+(k-2)\delta}$,
with each query requiring $O(\log n)$ rounds to evaluate.
Taking $\delta = (k-2)/(k(k-1))$,
we get a running time of 
$\tilde{O}(n^{1/2 - 1/(2k(k-1))})$.



%\subsection{Heavy Cycle Procedure (any constant $k \geq 2$)}
%Let $V_h = \{v | d(v) \geq n^\delta\}$ be the set of ''heavy nodes''. First, the network counts the number of ''heavy'' nodes $|A|$, and each node in $A$ is assigned a unique number in $[|V_h|]$. Each node $v$ not in $V_h$ assigns itself a uniformly random color $c(v) \in [2k-1]$, and all nodes in $V_h$ assign themselves the color $2k$. For $i=1,\dots,|V_h|$, we define the protocol $A_i$ as follows: the $i$'th node in $V_h$ sends its id to all its neighbors. Following this, iteratively for $j=1,\dots,k-1$, nodes with color $k-i$ and $k+i$ sends the identifier it received by neighbors with color $k-i+1$, $k+i-1$ respectively to all their neighbors.  Finally, if a node with color $0$ received the same identifier from a neighbor with color $1$ and color $2k-1$, outputs that the graph is not $C_{2k}$-free.

%Using $v^*$ as a leader, the graph performs a Grover search as described in Lemma~\TODO{ref}, to find an $i \in \sqrt{n}$ for which the protocol $A_i$ rejects, or determines that there is no such $i$. We repeat this protocol $O(k^k)$ times; If in one of the instances of the protocol there is such an $i$, the network outputs that the graph is not $C_{2k}$-free, and otherwise it outputs that it is $C_{2k}$-free.

%\subsection{Light Cycle Procedure}
%Let $c_k > 0$ be a constant such that any $C_{2k}$-free graph has arboricity at most $c_kn^{1+1/k}$ First, the network attempts to compute a $c_kn^{1+1/k}$-forest decomposition using the procedure of \TODO{reference}. If the network fails, the network outputs that the graph is not $C_{2k}$-free. 
%
%Otherwise, each node $v$ assigns itself a uniformly random color $c(v) \in [2k]$, and a uniformly random set number $S(v) \in [\sqrt{n}]$. For $i=1,\dots,n^\delta$, we define the protocol $A_i$ as follows: each node $v$ with color $k$ and set number $i$ sends its id to all its neighbors. Following this, iteratively for $j=1,\dots,k-1$, nodes with color $k-i$ and $k+i$ send all the identifiers received by outgoing neighbors with color $k-i+1$, $k+i-1$ respectively to all their neighbors, assuming this set is not larger than $O(\log{n})$. Finally, if a node with color $0$ received the same identifier from a neighbor with color $1$ and color $2k-1$, outputs that the graph is not $C_{2k}$-free.
%
%Using $v^*$ as a leader, the graph performs a Grover search as described in Lemma~\TODO{ref}, to find an $i \in \sqrt{n}$ for which the protocol $A_i$ rejects, or determines that there is no such $i$. We repeat this protocol $O(k^k)$ times; If in one of the instances of the protocol there is such an $i$, the network outputs that the graph is not $C_{2k}$-free, and otherwise it outputs that it is $C_{2k}$-free.



%\subsection{Round Complexity}
%Setting $\delta = 1/(k-1)$, we get that the round complexity of the light cycle procedure is $\tilde{O}(\sqrt{n^{(k-2)\delta+1/k}\log{n}}) = \tilde{O}(\sqrt{n^{1-\frac{1}{k(k-1)}}}) = \tilde{O}(n^{1/2-\frac{1}{2k(k-1)}})$. On the other hand, by Markov's inequality \TODO{expand}, $|V_h| \leq n^{1+1/k-\delta}$. Therefore the heavy cycle procedure takes $\tilde{O}(\sqrt{n^{1+1/k-\delta}}) = \tilde{O}(n^{1/2-\frac{1}{2k(k-1)}})$ rounds.

%\subsection{Heavy Cycle Procedure (for $k = 2,3,4,5$)}
%\begin{lemma}[Implicit in \TODO{cite}]
	%For any parameter $\delta > 0$, There is a deterministic $O(1)$ round algorithm in $\CONGEST$ which is given as input a network with a single marked node, and has the following properties: If $G$ has a cycle with a node of degree at least $n^\delta/3$, then there is a set $S \subseteq V$ of size at least $n^\delta/2$ such that given a vertex $v \in S$, the algorithm outputs a $2k$-cycle.
	%\label{lem:small_heavy_cycles}
%\end{lemma}

%Applying a Grover search on all vertices with degree \TODO{complete}
%}





==> app_prelims.tex <==
\section{Extended Preliminaries and Missing Proofs}
\iffalse
\subsection[$k$-wise independent hash functions]{{\boldmath $k$}-wise independent hash functions}
For two integers $a,b$ we say that a function $f:[a]\rightarrow[b]$ is a $k$-wise independent hash function if for any $k$ distinct elements $x_1,\dots,x_k \in [a]$ and any $k$ elements $y_1,\dots,y_k \in [b]$, $\Pr(x_1 = y_1 \land \dots \land x_k = y_k) = 1/b^k$.

We cite a tail bound that is useful for bounding the size of a given bin in a $k$-wise independent hash functions.

\begin{lemma}[\cite{SJSS93},Theorem 5(II)(b)]
	\label{thm:tail_bound}
	If $\rv{X}$ is the sum of $k$-wise independent random variables,
	each of which is confined to the interval $[0,1]$ and has $\mu = E[\rv{X}]$,
	then for $\alpha \geq 1$ and assuming $k \leq \lceil \alpha \mu e^{-1/3} \rceil$,
	\begin{equation*}
	\Pr(|X-\mu| \geq \alpha \mu) \leq e^{-\lfloor k/2 \rfloor}.
	\end{equation*}
\end{lemma}
\fi



\subsection{Missing proofs}
\label{app_sec_prelims_proofs}

\begin{claim-repeat}{claim:batchMessaging}
	\ClaimBatch
\end{claim-repeat}

\begin{proof}[Proof of Claim~\ref{claim:batchMessaging}]
	We define a packet as a tuple $(m_i,k)$ where $m_i$ is a message of size $O(\log{n})$ and $k$ is an integer which represents a number of times this message needs to be duplicated. Throughout this procedure each node maintains a set of packets, where at the start it has for each message $m_i^v$, a packet $(m^v_i,|U^v_i|)$.The network repeats the following procedure for $i=1,\dots,\log{n}$ times: For $O(\mix)$ rounds, each node chooses for each packet a uniformly random incident edge, and assuming at most $O(\log^2{n})$ packets chose that edge, it sends the packet through that edge (which can be done in $\tilde{O}(1)$ rounds). After $O(\mix)$ rounds, if the number of packets on a node $v$ is at most $c\deg(v)\log^3{n}$ for a sufficiently large $c > 0$, we split each of its packets $(m,k)$ with $k > 1$ into two packets $(m,\lceil k \rceil)$ and $(m,\lfloor k \rfloor)$. We note that indeed there can be at most $2L|E|$ packets as the total load is at most $2L|E|$, and  the number of packets on each node at the end of an iteration is ${O}(L\deg(v)\log^2{n})$ w.h.p., and after splitting the messages, the number of packets at most doubled. By the latter property, with high probability after each iteration, every packet is split, implying that after iteration $i=\log{n}$ each packet has $k=1$ w.h.p.. In parallel for all node, for each message $m$ in a packet a node $v$ has after the final iteration, it chooses a node $u \in U_i^v$ uniformly at random, and using the routing scheme of Theorem~\ref{thm-expander-routing}, routes the message to $u$, which can be performed in $\tilde{O}(\mix)$ rounds for all messages.
\end{proof}

\iffalse
\begin{claim-repeat}{claim:2hopNeighborhood}
	\ClaimTwoHop
\end{claim-repeat}

\begin{proof}[Proof of Claim~\ref{claim:2hopNeighborhood}]
	Let $v$ be such a node. Node $v$ iterates over its at most $\alpha$ neighbors. When it considers neighbor $i$, it sends a message to all its neighbors asking if they neighbor $i$, to which they each respond whether or not they have an edge to node $i$. At the end of the iterations, after $O(\alpha)$ rounds, node $v$ knows all of its induced $2$-hop neighborhood.
	
	Notice that it does not matter if $v$ has a neighbor $u$ which also tries to perform this search in parallel to $v$, in the odd rounds $v$ and $u$ just sends queries to each other across their shared edge, and in the even rounds they each respond to one another.
\end{proof} 
\fi

==> introduction-old.tex <==
% !TEX root = ./main.tex
%====================
\section{Introduction}
%====================
\noindent{\bf Background.}
In the past few years there has been a surge of works investigating the complexity of the subgraph detection problem, which asks to detect the existence of a specified subgraph within the input graph, in the \congest and \clique models of distributed computing (in the \congest model the input graph coincides with the communication network). Most of these works, in particular, have focused on detecting $p$-cliques (denoted below $K_p$) and $\ell$-cycles (denoted below $C_\ell$), for small values of~$p$ and $\ell$.

%\noindent\textbf{Detecting cliques and cycles in the \congest model.}
In the \congest model, the first sublinear algorithm for $p$-clique detection was obtained for $p=3$ (i.e., triangle detection) by Izumi and Le Gall~\cite{ILG2017}. The complexity of triangle detection was then improved to $\tilde{O}(\sqrt{n})$ by Chang et al.~\cite{CPZ19}, where $n$ denotes the number of nodes, and then further to $\tilde{O}(n^{1/3})$ by Chang and Saranurak~\cite{CS19}. For $p$-cliques with $p\geq 4$, the first sublinear detection algorithm was constructed by Eden et al.~\cite{EFFKO19}. %, who showed the upper bounds $\tilde{O}(n^{5/6})$ rounds for $k=4$ and $\tilde{O}(n^{21/22})$ rounds for $k=5$.
These results were improved to $\tilde{O}(n^{p/(p+2)})$ rounds for all $p\geq 4$ by Censor-Hillel et al.~\cite{CHLGL20}, and very recently, $\tilde{O}(n^{1-2/p})$ rounds for all $p\geq 4$ by Censor-Hillel et al.~\cite{Censor+SODA21}. Czumaj and Konrad \cite{CK20} have shown the lower bound $\Omega(\sqrt{n})$ for $p$-clique detection for $p\ge 4$, which matches the upper bound from \cite{Censor+SODA21} for $p=4$. Proving lower bounds for triangle detection, on the other hand, appears extremely  challenging: it is known that for any $\varepsilon > 0$, showing a lower bound of $\Omega(n^{\varepsilon})$ on triangle detection implies strong circuit complexity lower bounds~\cite{CHFGLGDR20} (see nevertheless \cite{ACHKL20} for a weaker, but still non-trivial, lower bound for triangle detection).\footnote{Note that the algorithms from \cite{CPZ19,CHLGL20,CS19,Censor+SODA21} actually solve the listing version of the problem (which asks to list all $p$-cliques of the graph) as well. For the listing version, lower bounds matching the upper bounds from \cite{CS19,Censor+SODA21} for all values of $p\ge 3$ are known \cite{ILG2017,PS18,FGKO18}.} 

Concerning $\ell$-cycle detection in the \congest model, for odd $\ell\ge 5$ the complexity of the problem is known to be $\tilde{\Theta}(n)$ \cite{DKO14,KR17}. For $\ell=4$, Drucker et al.~\cite{DKO14} showed that the complexity is $\tilde \Theta(\sqrt{n})$. For even $\ell\ge 6$, Korhonen and Rybicki~\cite{KR17} showed a $\tilde{\Omega}(\sqrt{n})$ lower bound.  Fischer et al.~\cite{FGKO18} showed an $\tilde{O}(n^{1-1/(k^2-k)})$-round algorithm for $C_{k}$ detection for any $k\ge 3$, which was improved by Eden et al.~\cite{EFFKO19} to $\widetilde{O}(n^{1-2/(k^2-k+2)})$ for odd $k$ and $\widetilde{O}(n^{1-2/(k^2-2k+4)})$ for even $k$. Recently, Censor-Hillel et al.~\cite{CHFGLGDR20} showed that for $3\leq k \leq 5$, $C_{2k}$ detection can be solved in $\tilde{O}(n^{1-1/k})$ rounds. 

In the powerful \clique model, the best known upper bounds on the round complexity of $p$-clique detection is $O(n^{0.158})$ for $p=3$, which is obtained by the algebraic approach based on matrix multiplication developed by Censor-Hillel et al.~\cite{CHKKLPJ19}, and $O(n^{1-2/p})$ for any constant $p\ge 4$ \cite{DLP12}. For any even constant $\ell$, $\ell$-cycle detection can be solved in $O(1)$ rounds~\cite{CHFGLGDR20}. For any odd constant $\ell\geq 3$, the best known upper bound for $\ell$-cycle detection in the \clique model is $O(n^{0.158})$ rounds, obtained again by the algebraic approach from \cite{CHKKLPJ19}.\vspace{2mm}

\noindent{\bf Quantum distributed computing.}
The power of quantum computing in the distributed setting has also been the subject of intensive investigations recently. In quantum distributed computing, the main difference with classical (i.e., non-quantum) distributed computing is that quantum information, i.e., quantum bits (qubits), can be sent through the edges of the network instead of classical information, i.e., bits. Le Gall and Magniez \cite{LeGall+PODC18} have shown that for computing the diameter of the network, the quantum version of the \congest model (called below the \qcongest model), in which each vertex can send one message of $O(\log n)$ qubits to each adjacent vertex per round, is more powerful than the classical \congest model. 
%: they constructed a $\tilde{O}(\sqrt{n})$-round quantum algorithm for the exact computation of the diameter of the network (here~$D$ denotes the diameter), while it is known that any classical algorithm in the \congest model requires~$\tilde{\Omega}(n)$ rounds, even for graphs with constant diameter~\cite{FHW12}. 

Izumi et al. \cite{ILM20} recently showed an advantage for triangle detection as well, by constructing a quantum algorithm with round complexity $\tilde O(n^{1/4})$ in the \qcongest model (as mentioned above, the best known classical algorithm for triangle detection has complexity $\tilde O(n^{1/3})$). 
Note that achieving quantum speedups in the distributed setting is especially challenging since, as shown by Elkin et al.~\cite{EKNP14}, the ability to send quantum information is not helpful for many crucial components of distributed algorithms (e.g., routing or broadcast of information).
The key technique used in \cite{ILM20} is \emph{distributed Grover search}, which was introduced in \cite{LeGall+PODC18} and consists in a distributed implementation of Grover's celebrated quantum algorithm \cite{Grover96}.
\vspace{2mm}

\noindent{\bf Our results.} In this paper we investigate the power of quantum distributed algorithms for $p$-clique and $p$-cycle detection, in both the \qcongest model and the \qclique model. Using a new approach based on \emph{nested} distributed Grover searches, we obtain quantum algorithms that outperform their classical counterparts and in some cases go well below their lower bounds.

We first consider clique detection in the \qclique model. Our results are summarized in the following theorem (the upper bounds we obtain for $K_p$ detection with $p\ge 5$ are actually even stronger --- see Theorem \ref {thm:newCCextend} in Section \ref{sec:CC}).
\begin{theorem}\label{th:clique-clique}
There exists a quantum algorithm that solves $p$-clique detection with success probability at least $1-1/\poly(n)$ in the \qclique model with complexity $\tilde O(n^{1/5})$ for $p=3$, $\tilde O(n^{1/3})$ for $p=4$ and  $\tilde O(n^{1-2/(p-1)})$ for $p\ge 5$.
\end{theorem}

For all values $p\ge 2$, the quantum algorithms we obtain by Theorem \ref{th:clique-clique} are faster than all known classical and quantum algorithms for $p$-clique detection.
%. In particular, for triangle detection, it improves the $\tilde O(n^{1/4})$ upper bound from \cite{ILM20}. 

We then investigate clique detection in the \qcongest model.
% and obtain the following results.
\begin{theorem}\label{th:clique-congest}
There exists a quantum algorithm that solves $p$-clique detection with success probability at least $1-1/\poly(n)$ in the \qcongest model with complexity $\tilde O(n^{1/5})$ for $p=3$,
%, $\tilde O(n^{4/9})$ for $p=4$ and
and $\tilde O(n^{1-2/(p-1)})$ for $p\ge 7$.%\ftodo{Should we write the same value as in the classical case for $p=5$ and $p=6$?}
\end{theorem}

For all $p=3$ and $p\ge 7$, the quantum algorithms we obtain by Theorem~\ref{th:clique-congest} are faster than all known algorithms for $p$-clique detection in the \congest or \qcongest model.
%For $p=4$, the complexity in the \qcongest model even goes below the $\Omega(\sqrt{n})$-round lower bound in the classical \congest model by Czumaj and Konrad \cite{CK20}.
On the other hand, for $4 \leq p \leq 6$, our approach currently does not lead to any improvement over the complexities of the classical algorithms from \cite{Censor+SODA21}, which are respectively $\tilde O(\sqrt{n})$, $\tilde O(n^{3/5})$ and $\tilde O(n^{2/3})$. 
The reason is, informally, that in the $\qcongest$ model we (and all prior work on listing cliques)
decompose the graph into well-connected clusters, and simulate the $\qclique$ on each cluster;
for very small cliques, the effort required to collect the edges needed at each cluster overwhelms any time savings
we currently gain from the quantum search.
%\rtodo{Someone read the new explanation above and make sure it'sOK}

%, in both the \congest and the \clique models. Moreover, for triangle detection, our results improve the $\tilde O(n^{1/4})$ upper bound from \cite{ILM20}. 

We then consider cycle detection. Since efficient classical algorithms already exist in the \clique model (especially for even-length cycles), we mainly focus on cycle detection in the \qcongest model. Our main results are summarized in the following two theorems.

\begin{theorem}\label{th:cycle-odd}
For any odd constant $\ell\ge 3$, the complexity of $\ell$-cycle detection in the \qcongest model is $\tilde \Theta(\sqrt{n})$ rounds. 
\end{theorem}

\begin{theorem}\label{th:cycle-even}
%For any even constant $k\ge 3$, there exists a quantum algorithm that solves $2k$-cycle detection with success probability at least $1-1/\poly(n)$ in $\tilde O(n^{1/2-1/(2k(k-1))})$ rounds in the \qcongest model. 
	For any constant 
	$k \geq 2$,
	there is a $\QCONGEST$ algorithm that runs in $\tilde{O}(n^{1/2 - 1/(2k(k-1))})$
	rounds, and solves $C_{2k}$ detection with probability $1 - 1/\mathrm{poly}(n)$.
	\label{thm:C2k}
\end{theorem}
For all values $\ell\ge 3$, the quantum algorithms we obtain by Theorems~\ref{th:cycle-odd} and \ref{th:cycle-even} are faster than all known algorithms for $\ell$-cycles detection in the \congest model.

%\ftodo{Say a few words about the barrier results.}\otodo{Added a short paragraph}
Finally, we show a barrier for proving an $\Omega(n^{3/5+\epsilon})$ lower bound for $K_p$ detection for any $\eps > 0$. Namely, such a bound would imply breakthrough results in the field of circuit complexity, which are far beyond the current state-of-the-art.
\begin{theorem}[Informal]
	 For any constant integer $p \geq 4$ and any constant $\epsilon > 0$, proving a lower bound of $\Omega(n^{3/5+\epsilon})$ on $K_p$ detection for randomized $\CONGEST$ algorithms would imply new lower bounds on high-depth circuits with constant fan-in and fan-out gates.
	\label{thm:Kp_obstacle}
\end{theorem}

Previously, several such barriers were known: in \cite{EFFKO19} it is shown that there is an absolute constant $c$ such that proving a lower bound of the form $\Omega(n^{1-c})$ for $C_{2k}$ detection would imply breaking a circuit complexity barrier. In \cite{EFFKO_note} such a barrier is shown for proving an $\Omega(n^\epsilon)$ lower bound on triangle detection, and in \cite{CHFGLGDR20} a barrier for proving a lower bound of $\Omega(n^{1/2+\epsilon})$ for $C_6$ detection is given.

We refer to Table \ref{table:results} for a summary of our results and a detailed comparison with prior works.%\ftodo{I am not sure if this really makes sense to have a table. If we can't display nicely our results in the table, let's remove it.}\dtodo{We can perhaps display in a line--graph, with the $x$-axis being the clique size, and the $y$-axis being the complexity} 
\vspace{2mm}
\begin{table}[tb]\centering
  \caption{Our upper bounds for subgraph detection, and the corresponding known results in the classical setting. Here $n$ denotes the number of nodes in the network. For even-length cycle detection the table also shows the concrete upper bounds given by Theorem~\ref{th:cycle-even} for $k=2,3,4,5$.}
  \begin{tabular}{|p{2.3cm}|p{3.3cm}|p{4.5cm}|} \hline
    Subgraph & \clique & \qclique \\ \hline \hline
    \multirow{2}{*}{$K_3$}&\multirow{2}{*}{$\tilde{O}(n^{1/3})$\,\hspace{14mm} \cite{CS19}}& $\tilde{O}(n^{1/4})$ \bigstrut \hspace{17mm}\cite{ILM20}\\
                                       && $\tilde{O}(n^{1/5})$\hspace{16mm}  Theorem~\ref{th:clique-clique} \\ \hline
    $K_4$& $\tilde{O}(\sqrt{n})$\bigstrut\hspace{15mm}\: \cite{Censor+SODA21}& $\tilde{O}(n^{1/3})$\hspace{16mm}  Theorem~\ref{th:clique-clique} \\ \hline
    $K_p$ ($p\ge 5$)& $\tilde{O}(n^{1-2/p})$\bigstrut\hspace{11mm} \cite{Censor+SODA21}& $\tilde{O}(n^{1-2/(p-1)})$  \hspace{6mm}  Theorem~\ref{th:clique-clique}\\ \hline
  \end{tabular}
\vspace{4mm}

  \begin{tabular}{|p{2.3cm}|p{3.3cm}|p{4.5cm}|} \hline
    Subgraph & \congest & \qcongest \\ \hline \hline
    \multirow{2}{*}{$K_3$}&\multirow{2}{*}{$\tilde{O}(n^{1/3})$\,\hspace{14mm}\cite{CS19}}& $\tilde{O}(n^{1/4})$\bigstrut  \hspace{17mm}\cite{ILM20}\\
                                       && $\tilde{O}(n^{1/5})$  \hspace{15mm}  Theorem~\ref{th:clique-congest} \\ \hline
    %$K_4$& $\tilde{\Theta}(\sqrt{n})$\bigstrut\:\hspace{14mm} \cite{Censor+SODA21,CK20}& $\tilde{O}(n^{4/9})$  \hspace{15mm}  Theorem~\ref{th:clique-congest} \\ \hline
    $K_p$ ($p\ge 7$)& $\tilde{O}(n^{1-2/p})$\bigstrut\hspace{11mm}\cite{Censor+SODA21}& $\tilde{O}(n^{1-2/(p-1)})$  \hspace{6mm}  Theorem~\ref{th:clique-congest} \\ \hline\hline
   $C_\ell$ ($\ell\ge 5$ odd)& $\tilde{\Theta}(n)$\bigstrut\:\hspace{18mm}\cite{DKO14}& $\tilde{\Theta}(\sqrt{n})$  \hspace{16mm}  \:Theorem~\ref{th:cycle-odd} \\ \hline
   $C_\ell$ ($\ell\ge 4$ even)& $\tilde{O}(n^{1-1/\Theta(\ell^2)})$\bigstrut\:\hspace{5mm}\cite{EFFKO19}& $\tilde{O}(n^{1/2-1/\Theta(\ell^2)})$  \:\hspace{3mm}  Theorem~\ref{th:cycle-even} \\ \hline
$C_4$ & $\tilde{\Theta}(\sqrt{n})$\hspace{16mm}\cite{DKO14}\bigstrut& $\tilde{O}(n^{1/4})$  \hspace{15mm}  Theorem~\ref{th:cycle-even} \\ \hline
$C_6$ & $\tilde{O}(n^{2/3})$ \,\hspace{12mm} \cite{CHFGLGDR20}\bigstrut& $\tilde{O}(n^{5/12})$  \!\hspace{14mm}  Theorem~\ref{th:cycle-even} \\ \hline
$C_8$ & $\tilde{O}(n^{3/4})$ \,\hspace{12mm} \cite{CHFGLGDR20}\bigstrut& $\tilde{O}(n^{11/24})$  \!\hspace{13mm}  Theorem~\ref{th:cycle-even} \\ \hline
$C_{10}$ & $\tilde{O}(n^{4/5})$ \,\hspace{12mm} \cite{CHFGLGDR20}\bigstrut& $\tilde{O}(n^{19/40})$  \!\hspace{13mm}  Theorem~\ref{th:cycle-even} \\ \hline
  \end{tabular}\label{table:results}
\end{table}


\noindent{\bf Overview of our main technique.}
The main technical tool used to design our quantum algorithms is the framework of distributed Grover search developed in \cite{LeGall+PODC18}, which can be described as a distributed implementation of Grover's quantum algorithm \cite{Grover96}. Grover's algorithm consists of an alternation of quantum operations (called Grover diffusion operations) and checking operations (also called checking queries). 
In the distributed implementation developed in \cite{LeGall+PODC18}, one specific node of the network (the leader) executes each Grover diffusion operation locally, but implements each query in a distributed way using a distributed checking procedure. While all prior works using this framework (\!\!\cite{Izumi+PODC19, LeGall+PODC18,ILM20}) considered the setting where the checking procedure is a classical procedure, in this work we also consider checking procedures that themselves also apply distributed quantum searches. We develop a framework to describe such ``nested'' quantum searches (see Lemma \ref{lemma:qsearchv1} and \ref{lemma:qsearch} in Section~\ref{section:prelim}). Our framework can actually be applied in a completely ``black-box'' way to design quantum distributed algorithms (i.e., no knowledge of quantum computation is needed to apply this framework).

Our results on $K_p$-detection (Theorems \ref{th:clique-clique} and \ref{th:clique-congest}) are obtained by combining this framework for nested quantum searches with the techniques introduced in prior works on classical clique-detection algorithm \cite{ILG2017, CPZ19, CS19,CHLGL20,Censor+SODA21}.  Even with our new framework, achieving quantum speedups for these classical algorithms is nevertheless far from being straightforward since, as already mentioned, the ability to send quantum information is not helpful for many crucial components of distributed algorithms. We end up having to  modify the approach taken in those prior works and tailor it to our needs. We develop a new approach for detecting cliques, by first classically listing all instances of some smaller-sized clique, and then using nested quantum search to search for an extension into a larger clique. We actually give two variations of this approach, and use them to obtain improved algorithms for both the \qclique model (Section \ref{sec:CC}) and the \qcongest model (Section \ref{sec:qcongest}).

Our results on $C_\ell$-detection (Theorems~\ref{th:cycle-odd} and \ref{th:cycle-even}) are obtained by applying distributed Grover search on the state-of-the-art classical distributed algorithms for $C_\ell$-detection \cite{CHFGLGDR20,DKO14,EFFKO19,FGKO18}. 
 \vspace{2mm}

\noindent{\bf Further related works on quantum distributed computing.}
There exist a few works investigating the power of quantum distributed computing in other models  or settings (see also \cite{Arfaoui+14} and \cite{Denchev+08} for surveys). 
%The quantum version of the \congest model (called below the \qcongest model), in which each vertex can send one message of $O(\log n)$ qubits  to each adjacent vertex per round, was first be investigated by Elkin et al.~\cite{EKNP14}. Their discoveries were nevertheless negative: they showed that for many important graph-theoretical problems, the ability to send quantum information is not helpful. 
In the \clique model, Izumi and Le Gall~\cite{Izumi+PODC19} showed that quantum distributed algorithms can also be more powerful than classical distributed algorithms: they constructed a quantum algorithm faster than the best known classical algorithms for the All-Pair Shortest Path problem.
In the \local model, separations between the computational powers of the classical and quantum algorithms have been also obtained \cite{GKM09,LNR19}. Over anonymous networks, zero-error quantum algorithms have been constructed for leader election \cite{Tani+12}. Finally, quantum algorithms for byzantine agreements have also been investigated \cite{Ben-Or+STOC05}.


==> quantum_cycle.tex <==
\section{Fast Quantum Algorithm for {\boldmath $C_{\ell}$}-Freeness}
\label{sec:cycles}

In this section we give quantum $\CONGEST$ algorithms for solving the $C_{\ell}$-freeness problem (i.e., $C_{\ell}$-detection) for constant $\ell$.
For odd-length cycles, 
there is a very simple algorithm that runs in $\tilde{O}(\sqrt{n})$ rounds:
essentially, we use Grover search to check if there is a vertex $\tilde{v} \in V$
such that an $O(\ell)$-round BFS starting from $\tilde{v}$ finds an $\ell$-cycle in which $\tilde{v}$
participates.
Since we think of $\ell$ as a constant, the running time of the entire search is $\tilde{O}(\sqrt{n})$.
\begin{theorem}
	For any odd length $\ell \geq 5$,
	the $C_{\ell}$-freeness problem can be solved in $\tilde{O}(\sqrt{n})$ rounds in $\QCONGEST$,
	with success probability $1 - 1/\mathrm{poly}(n)$.
	\label{thm:Codd}
\end{theorem}
In Appendix~\ref{app:cycles:odd} we give more details,
and also show the following lower bound, implying that the above complexity is optimal up to polylogarithmic factors. Theorems \ref{thm:Codd} and \ref{thm:Codd-lb} together give Theorem \ref{th:cycle-odd} stated in the introduction.


\newcommand{\OddCycleLB}
{
	For any odd length $\ell \geq 5$,
	the $C_{\ell}$-freeness problem requires $\tilde{\Omega}(\sqrt{n})$ rounds in $\QCONGEST$.
}
\begin{theorem}
	\label{thm:Codd-lb}
	\OddCycleLB
\end{theorem}


For even-length cycles, $\ell = 2k$,
we give a more complex algorithm that runs in $o(\sqrt{n})$ rounds.
The algorithm follows the general outline of the algorithms from \cite{FGKO18,EFFKO19}: it first searches for cycles containing some high-degree node (``heavy cycles''), and then, if no such cycle is found, it removes all high-degree nodes from consideration, and searches for cycles containing only low-degree nodes (``light cycles''). We show that using quantum search, we can search for both heavy and light cycles more quickly than the best-known classical equivalent. Specifically, in the case of 4-cycles, there is a classical lower bound of $\tilde{\Omega}(\sqrt{n})$ rounds \cite{DKO14}, while our quantum algorithm runs in $\tilde{O}(n^{1/4})$ rounds. This shows another separation between the classical and quantum distributed models.

\subparagraph{Searching for heavy cycles.}
Let us say that a cycle is \emph{heavy} if it contains some node of degree $\geq n^{\delta}$.
The procedure we use to search for heavy cycles is the same as the one used in Theorem~\ref{thm:Codd}:
we simply user Grover search to check, using (slightly modified) BFS,
whether there is a node with degree $\geq n^{\delta}$ that participates in a $2k$-cycle.
Unlike the case of odd cycles, here we can also use the fact that any graph that is $C_{2k}$-free
has at most $O(n^{1+1/k})$ edges; thus, the number of nodes with degree $\geq n^{\delta}$
is bounded by $O(n^{1+1/k - \delta})$, and we can search over them in $\tilde{O}(n^{(1+1/k-\delta)/2})$ rounds using Grover search.
Following this step, we remove all nodes with degree $\geq n^{\delta}$ from consideration.
 
\subparagraph{Searching for light cycles.}
In~\cite{FGKO18,EFFKO19}, light cycles are found by relying on the fact that a $C_{2k}$-free graph not only has at most $O(n^{1+1/k})$ edges, it also has arboricity (a notion of ``hereditary average degree'') at most $O(n^{1/k})$. 
We search for light cycles by having many nodes start a BFS at the same time, using the bounded arboricity and the maximum degree of $n^{\delta}$ to manage the search in such a way that no node needs to forward more than $O(n^{1/k+(k-2)\delta})$ BFS tokens.

The key idea for speeding up this part of the algorithm is to partition the BFS sources into small sets, by randomly assigning each BFS source an index in $[n^{1/k + (k - 2)\delta}]$.
We use Grover search over the indices to check if for some index $i$, there is a BFS source with index $i$ that participates in a $2k$-cycle.
The number of BFS tokens \emph{with the same index} that reach a given node is now bounded by $O(1)$ in expectation,
so the entire search requires $\tilde{O}(n^{(1/k+(k-2)\delta)})$ rounds.

Balancing the running time of the two parts of the algorithm (heavy cycles and light cycles) yields the final running time of $\tilde{O}(n^{1/2-\Theta(1/k^2)})$.




==> sparse.tex <==
%======================================
% \section{A \qclique algorithm for detecting $K_p$}
\section{Sparsity-Aware Detection in the $\qclique$ Model}
\label{sec:sparseCC}
%======================================
Here we show a \emph{sparsity-aware} version of detecting cliques in the \qclique model. That is, if the input graph is sparse, our algorithm is faster. The key realization is that information regarding $\Theta(n)$ edges can be broadcast in the \clique model in $O(1)$ rounds, thus, enabling one to coalesce the checking of several nodes at once. This in turn changes the dependency of the round complexity from the number of nodes in the graph, $n$, to the average degree in the graph, $\mu = \Theta(m/n)$. Formally, we prove the following.


%Using Theorem~\ref{extendingTheoremSparsityAware}, it is possible to show a sparsity aware version of the above.

\begin{theorem}
\label{th:sparseCC}
	Given a graph $G = (V, E)$, and some value $p$, it is possible to detect whether there exists an instance of $K_p$ in $G$ within $\tilde{O}(\min_{\ell \in \mathbb{N}} \max \{m / n^{1+\frac{2}{p-\ell}}, (m/n)^{1-\frac{1}{2^\ell}}\})$ rounds of the \qclique model.
\end{theorem}


\ktodo{Be consistent with $m/n$ vs $\mu$. Either have both theorems be in terms of $m/n$ (and then maybe use $(m/n)^{...}$ instead of $m/n^{....}$) or in terms of $\mu$ (and then say in the statements that this is the average degree.)}


%Here we show a \emph{sparsity-aware} version of Theorem~\ref{extendingTheorem}. The key realization is that information regarding $\Theta(n)$ edges can be broadcast in the \clique model in $O(1)$ rounds, thus, enabling one to coalesce the checking of several nodes at once. This in turn changes the dependency of the round complexity from the number of nodes in the graph, $n$, to the average degree in the graph, $\mu = \Theta(m/n)$. 

To prove Theorem~\ref{th:sparseCC}, we show that we can detect a $K_{p + t}$ instance from $K_p$-listing, in a sparsity-aware manner. This is an analogue to Theorem~\ref{extendingTheorem}.
\begin{theorem}
	\label{extendingTheoremSparsityAware}
	Given a graph $G = (V, E)$ and values $p$, $t$. Assuming that every instance of $K_p$ is known to some node, then it is possible to detect if $G$ contains an instance of $K_{p + t}$ in $\tilde{O}(\mu^{1-\frac{1}{2^t}})$ rounds of communication in the \qclique, w.h.p. 
\end{theorem}

Using Theorem~\ref{extendingTheoremSparsityAware} we can prove Theorem~\ref{th:sparseCC} as follows.

\begin{proof}[Proof of Theorem~\ref{th:sparseCC}]
	Fix $\ell \in \mathbb{N}$. Perform $K_{p-\ell}$ listing using the algorithm from \cite{CHLGL20} within $\tilde O(m/n^{1+\frac{2}{p-\ell}})$ rounds. Then, execute Theorem~\ref{extendingTheoremSparsityAware} within $\tilde O((m/n)^{1-1/2^{\ell}})$ rounds in order to detect the existence of an instance of $K_p$.
\end{proof}

It remains to prove Theorem~\ref{extendingTheoremSparsityAware}. 

\begin{proof}[Proof of Theorem~\ref{extendingTheoremSparsityAware}]
	Initially, we \emph{batch} together the nodes into sets such that the sum of the degrees of the nodes in each set is $\Theta(n)$. Clearly, by broadcasting the degree of each node, it is possible to partition the nodes into $V = Y_1 \cup \dots \cup Y_{y}$, where, for $i \in [y]$ the sum of the degrees in $Y_i$ is $\Theta(n)$, and $y = \Theta(m/n) = \Theta(\mu)$. Thus, within $1$ round, all nodes can locally compute such a partition. 
	
	Further, observe that for any single $i \in [y]$, it is possible in $O(1)$ rounds to broadcast the neighbors of every node in $Y_i$. To do so, every node in $Y_i$ broadcasts its degree, allowing all the nodes to locally \emph{assign} to every node $O(1)$ of the edges  incident to nodes in $Y_i$. Finally, as every node is assigned $O(1)$ edges, it broadcasts those edges in $O(1)$ rounds.
	
	Similarly to the $Y_i$ sets, we split $V$ into sets $X_{1}, \dots, X_{x}$, where $x = \mu^{1/2^{t-1}}$, ensuring that the sum of the degrees of the nodes in each set is $\Theta(m/x)$. Notice that similarly to the above, it is possible to broadcast the edges incident to all nodes in a specific $X_i$ in $O(m/xn) = O(\mu / x)$ rounds.
	
	Now, as in the proof of Theorem~\ref{extendingTheorem}, we proceed with proving the claimed complexity through an induction on $t$.\ktodo{The notation there is completely different. There are two more references below to claims in the proof of Theorem~\ref{extendingTheorem}, but this currently doesn't work.}
%\vspace{2mm}
	
%	\paragraph{Base case, $t= 1$.} 
\noindent{\bf Base case, {\boldmath $t= 1$}.}
Given that every instance of $K_p$ is known to some node, we desire to detect if there is an instance of $K_{p+1}$ in the graph, within $\tilde O(\mu^{1/2})$ rounds. To do so, we perform a quantum search over $y$, to look for $i \in [y]$ such that there exists $v^* \in Y_i$ where $v^*$  is in some instance of $K_{p+1}$. That is, fix $i \in [y]$, and, using the above, broadcast the edges incident to the nodes in $Y_i$. Then, every node broadcasts if it is aware of some $K_{p+1}$ or not. If there is a $\tilde{v} \in Y_i$ \ktodo{Is there a need here for a new notation $\tilde{v}$? The previous sentence used $v^*$ for the same thing, no?} and an instance of $K_{p+1}$ which includes $\tilde{v}$, denoted $\kappa = \{v_1, \dots, v_p, \tilde{v}\}$, then it is guaranteed that some node knows it, due to similar claims as in the proof of Theorem~\ref{extendingTheorem}.
	% Denote by $w$ the node which knows the instance of $K_p$, $\kappa \setminus \{\tilde{v}\}= \{v_1, \dots, v_p\}$. It is guaranteed that such a $w$ exists as we are given that all $K_p$ have been listed. Thus, as the edges incident to the nodes in $Y_i$, and hence $\tilde{v}$ have been broadcast, node $w$ sees $\kappa$ and reports to the entire graph that a $K_{p+1}$ exists. 
	Finally, we perform this quantum search over $[y]$, and so due to Lemma~\ref{lemma:qsearch}, this executes in $\tilde O(y^{1/2})$ rounds.\vspace{2mm}
	
	
%	\paragraph{Induction step, assuming correctness for $<t$.}  
\noindent{\bf Induction step, assuming correctness up to \boldmath{$t-1$}.}
We perform a quantum search over the sets $X_1, \dots, X_{x}$. Recall that $x = \mu^{1/2^{t-1}}$. Fix $i \in [\mu^{1/2^{t-1}}]$, and observe $X_i$. As before, broadcast the edges incident to nodes in $X_i$ within $\Theta(\mu / x) = \Theta(\mu^{1-1/2^{t-1}})$ rounds. Then, execute the algorithm for extending $K_{p+1}$ to $K_{p + t}$, by using $\tilde{t} = t-1$, within $\tilde O(\mu^{1-1/2^{\tilde{t}}}) = \tilde O(\mu^{1-1/2^{t-1}})$ rounds. Finally, as we perform a quantum search over $i \in [\mu^{1/2^{t-1}}]$, where each checking step requires $\tilde{O}(\mu^{1-1/2^{t-1}})$ rounds, the algorithm completes in $\tilde{O}(\mu^{1/2^{t}} \cdot \mu^{1-1/2^{t-1}}) =  \tilde{O}(\mu^{1-1/2^t}) $ rounds.\vspace{2mm}
	
	The correctness of the algorithm follows exactly from the same claims as in the proof of Theorem~\ref{extendingTheorem}.
	\end{proof} 

%To do so, we perform a Grover search over $V$, to look for a node $v^* \in V$ such that $v^*$ is in some instance of $K_{p+1}$. That is, fix $\tilde{v} \in V$, and every node $u \in V$ broadcasts if $\tilde{v}$ is its neighbor. Then, every node broadcasts if it is aware of some $K_{p+1}$ or not. If there is an instance of $K_{p+1}$ which includes $\tilde{v}$, denoted $\kappa = \{v_1, \dots, v_p, \tilde{v}\}$, then it is guaranteed that some node knows it. Denote by $w$ the node which knows the instance of $K_p$, $\kappa \setminus \{\tilde{v}\}= \{v_1, \dots, v_p\}$. It is guaranteed that such a $w$ exists as we are given that all $K_p$ have been listed. Thus, node $w$ would receive messages from each of $\kappa \setminus \{\tilde{v}\}$ telling it that they neighbor $\tilde{v}$, and so $w$ would see $\kappa$ and report to the entire graph that a $K_{p+1}$ exists. Finally, we perform this Grover search over $V$, and so due to Lemma~\ref{lemma:qsearch}, this executes in $\tilde O(n^{1/2})$ rounds.\vspace{2mm}

%\paragraph{Induction step, assuming correctness for $<t$.} 

%%%% NEW p -> p+t extension %%%%%%%%%%%%%%%%%
%\input{newccextend.tex}

